Causal Feature Selection via Orthogonal Search

The problem of inferring the direct causal parents of a response variable among a large set of explanatory variables is of high practical importance in many disciplines. However, established approaches often scale at least exponentially with the number of explanatory variables, are difficult to extend to nonlinear relationships, and are difficult to extend to cyclic data. Inspired by {\em Debiased} machine learning methods, we study a one-vs.-the-rest feature selection approach to discover the direct causal parent of the response. We propose an algorithm that works for purely observational data while also offering theoretical guarantees, including the case of partially nonlinear relationships possibly under the presence of cycles. As it requires only one estimation for each variable, our approach is applicable even to large graphs. We demonstrate significant improvements compared to established approaches.

==> TMLR 2022_ Causal Feature Selection via Orthogonal Search 2/algorithm.tex <==
\begin{algorithm*}[htb!]
\caption{Efficient Causal Orthogonal Structure Search (CORTH Features)}
\label{alg:double_ml_causal}
\begin{algorithmic}[1]
\STATE \textbf{Input:} response $Y \in \mathbb{R}^N$, covariates  $\mathbb{X}\in \mathbb{R}^{N \times d}$, significance level $\alpha$, number 
of partitions $K$.
%\EndIndent
\STATE Split $N$ observations into K random  partitions, $I_{k}$ for $ k = 1, \dots, K$, each having $n = N/K$ samples.
    \FOR{$i = 1,\dots,d$}
    \FOR{Subsample $k \in [K]$}
        \STATE $D_k\leftarrow X_i^{[k]}$ and $Z_k\leftarrow X_{\backslash i}^{[k]}$ \label{test}
        \STATE Fit $ m_{i}^{[\backslash k]}(Z_{\backslash k})$ to $D_{\backslash k}$ and  fit $g_{i}^{[\backslash k]}(Z_{\backslash k})$ to $Y^{[\backslash k]}$
        \STATE $\Hat{V}_{ij}^{[k]}\leftarrow D_{kj} -  m_{i}^{[\backslash k]}(Z_{kj})$, for all $j\in I_k$
        \STATE $\check{\theta}_i^{[k]} \leftarrow \big( \frac{1}{n} \sum_{j \in I_{k}} \Hat{V}_{ij}^{[k]} D_{kj} \big)^{-1}  \frac{1}{n} \sum_{j \in I_{k}} \Hat{V}_{ij}^{[k]} 
          (Y_{ij}^{[k]} - g_{ij}^{[\backslash k]}(Z_{kj})) $
        \STATE $ \hat{\chi}_i^{[k]} \leftarrow \frac{1}{n} \sum_{j \in I_{k}} \big( -Y_j^{[k]}m_{ij}^{[\backslash k]}(Z_{kj})  -
        D_{kj}g_{ij}^{[\backslash k]}(Z_{kj}) + m_{ij}^{[\backslash k]}(Z_{kj}) g_{ij}^{[\backslash k]}(Z_{kj}) 
          + Y_{j}^{[k]} D_{kj} \big) $
        \STATE $ (\hat{\sigma}_i^{[k]})^2 \leftarrow \frac{1}{n} \sum_{j \in I_{k}} \big( -Y_j^{[k]}m_{ij}^{[\backslash k]}(Z_{kj}) -
        D_{kj}g_{ij}^{[\backslash k]}(Z_{kj}) + m_{ij}^{[\backslash k]}(Z_{kj}) g_{ij}^{[\backslash k]}(Z_{kj})  + Y_{j}^{[k]} D_{kj} - \hat{\chi}_i^{[k]} \big)^2$
    \ENDFOR
    \STATE $ \hat{\theta}_i \leftarrow \frac{1}{K} \sum_{k \in K} \check{\theta}_i^{[k]}$, $ \hat{\chi}_i \leftarrow \frac{1}{K} \sum_{k \in K} \hat{\chi}_i^{[k]}$ \text{and } ${\hat{\sigma}_i}^2 \leftarrow \frac{1}{K} \sum_{k \in K} (\hat{\sigma}_i^{[k]})^2$ 
    \ENDFOR
    \FOR { $i \in [d]$}
        \STATE Gaussian normality test for $ \hat{\chi}_i \approx N\Big(0, \frac{{\hat{\sigma}_i}^2}{N} \Big)$ with $\alpha$ significance level and select $i^{\text{th}}$ feature if null-hypothese is rejected.
%        %\STATE Test for 0 mean of $\check{\theta}_i$
%        \IF{rejected}
%        \STATE $DecVec[i]=1$ 
%        \ELSE
%        \STATE $DecVec[i]=0$
%        \ENDIF
    \ENDFOR
\STATE \textbf{Return} Decision Vector
%\EndIndent
\end{algorithmic}
\end{algorithm*}

==> TMLR 2022_ Causal Feature Selection via Orthogonal Search 2/covid_tables.tex <==
\begin{table}[!htb]
    % \caption{Global caption}
    \begin{minipage}{.45\linewidth}
      \caption{Ranks of the features based on the times being predicted as direct causes of \textbf{SARS-Cov-2 exam result} out of 1000 different runs of our propsal approach. Not mentiond features were not predicted even once, note that preprocessed dataset has 331 features.}
      \label{Table:Covid_exam_result1}
        \resizebox{0.48\textwidth}{!}{\begin{minipage}{\textwidth}
        \begin{tabular}{ |c| l||c| }
         \hline  
         Rank & Feature & Rate of being Predicted as a Direct Cause \\ 
         \hline
         \hline
         \multirow{4}{*}{1} & Patient age quantile & \multirow{4}{*}{1} \\
        %  \hline
          & Arterial Lactic Acid &  \\
        %  \hline
          & Promyelocytes & \\
        %  \hline 
          & Base excess venous blood gas analysis &  \\
         \hline
         5 & pH venous blood gas analysis & 0.999 \\
         \hline
         6 & MISSING Mean platelet volume & 0.992 \\
         \hline
         7 & MISSING Lactic Dehydrogenase & 0.966 \\
         \hline
         8 & Segmented & 0.934 \\
         \hline
         9 & Myelocytes & 0.904 \\
         \hline
         10 & Eosinophils & 0.794 \\
         \hline
         11 & Leukocytes & 0.784 \\
         \hline
         12 & Total CO2 arterial blood gas analysis & 0.450 \\
         \hline
         13 & Potassium & 0.340 \\
         \hline
         14 & MISSING International normalized ratio INR & 0.289\\
         \hline
         15 & Metapneumovirus not detected & 0.234 \\
         \hline
         16 & Arteiral Fio2 & 0.092 \\
         \hline
         17 & HCO3 arterial blood gas analysis. & 0.046 \\
         \hline
         18 & Creatinine & 0.035 \\
         \hline
         19 & MISSING.Magnesium & 0.034 \\
         \hline
         20 & pO2 arterial blood gas analysis & 0.031 \\
         \hline
         21 & MISSING Arteiral Fio2 & 0.024 \\
         \hline
         22 & Direct Bilirubin & 0.016 \\
         \hline
         \multirow{2}{*}{23} & MISSING Ferritin & \multirow{2}{*}{0.014} \\
          & Respiratory Syncytial Virus detected & \\
          \hline
          \multirow{2}{*}{25} & MISSING Albumin & \multirow{2}{*}{0.010} \\
          & Creatine phosphokinase CPK & \\
         \hline
         27 & Strepto A positive & 0.008 \\
         \hline
         \multirow{4}{*}{28} & Neutrophils & \multirow{4}{*}{0.004} \\
          & Red blood cell distribution width RDW &  \\
         & Coronavirus HKU1 detected &  \\
         & Influenza A rapid test positive &  \\
         \hline
         32 & Hb saturation venous blood gas analysis & 0.002 \\
         \hline
         \multirow{5}{*}{33} & Urine pH & \multirow{5}{*}{0.001} \\
         & Inf A H1N1 2009 detected & \\
         & MISSING Serum Glucose & \\
         & Aspartate transaminase & \\
         & Urine Esterase nan & \\
         \hline
    \end{tabular}
    \end{minipage}}
    \end{minipage}%
    \hspace{1cm}
    \begin{minipage}{.45\linewidth}
        \vspace{-0.8cm}
        \caption[Caption for LOF]{Ranks of the features based on the times being predicted as direct causes of \textbf{Patient addmited to regular ward} out of 1000 different runs of our propsal approach. Not mentiond features were not predicted even once, note that preprocessed dataset has 331 features.}
	    \label{Table:Covid_exam_result2}
	    \resizebox{0.48\textwidth}{!}{\begin{minipage}{\textwidth}
        \begin{tabular}{ |c| l||c| }
         \hline  
         Rank & Feature & Rate of being Predicted as a Direct Cause \\ 
         \hline
         \hline
         \multirow{4}{*}{1} & Patient age quantile & \multirow{4}{*}{1} \\
        %  \hline
          & HCO3 venous blood gas analysis &  \\
        %  \hline
          & Total CO2 venous blood gas analysis & \\
        %  \hline 
          & Gamma glutamyltransferase &  \\
         \hline
         5 & MISSING Lactic Dehydrogenase & 0.987 \\
         \hline
         6 & Alanine transaminase & 0.845 \\
         \hline
         7 & MISSING International normalized ratio INR & 0.804 \\
         \hline
         8 & Serum Glucose & 0.652 \\
         \hline
         9 & pH venous blood gas analysis & 0.631 \\
         \hline
         10 & Base.excess venous blood gas analysis & 0.341 \\
         \hline
         11 & MISSING Arteiral Fio2 & 0.334 \\
         \hline
         12 & Urine Density & 0.334 \\
         \hline
         13 & Magnesium & 0.323 \\
         \hline
         14 & Metapneumovirus not detected & 0.261\\
         \hline
         15 & MISSING Mean platelet volume & 0.118 \\
         \hline
         16 & Creatine phosphokinase CPK & 0.086 \\
         \hline
         17 & Creatinine & 0.058 \\
         \hline
         18 & International normalized ratio INR & 0.049 \\
         \hline
         19 & MISSING Ferritin & 0.046 \\
         \hline
         20 & Urea & 0.044 \\
         \hline
         21 & Respiratory Syncytial Virus detected & 0.032 \\
         \hline
         22 & MISSING Magnesium & 0.021 \\
         \hline
         23 & MISSING Albumin & 0.018 \\
         \hline
         24 & MISSING Potassium & 0.016 \\
         \hline
         25 & Inf A H1N1 2009 detected & 0.014 \\
         \hline
         26 & Coronavirus HKU1 detected & 0.010 \\
         \hline
         27 & Strepto A positive & 0.008 \\
         \hline
         28 & Influenza A rapid test positive & 0.007 \\
         \hline
         \multirow{2}{*}{29} & MISSING Sodium & \multirow{2}{*}{0.002} \\
          & Urine Protein nan & \\
         \hline
         \multirow{3}{*}{31} & ctO2 arterial blood gas analysis & \multirow{3}{*}{0.001} \\
          & Influenza A detected & \\
          & Influenza B detected & \\
         \hline
    \end{tabular}
    \end{minipage}}
    \end{minipage} 
\end{table}

\begin{table}[!htb]
    % \caption{Global caption}
    \begin{minipage}{.45\linewidth}
    \vspace{-0.55cm}
      \caption[Caption for LOF]{Ranks of the features based on the times being predicted as direct causes of \textbf{Patient addmited to semi-intensive unit} out of 1000 different runs of our propsal approach. Not mentiond features were not predicted even once, note that preprocessed dataset has 331 features.}
	  \label{Table:Covid_exam_result3}
        \resizebox{0.48\textwidth}{!}{\begin{minipage}{\textwidth}
        \begin{tabular}{ |c| l||c| }
         \hline  
         Rank & Feature & Rate of being Predicted as a Direct Cause \\ 
         \hline
         \hline
         \multirow{7}{*}{1} & Patient age quantile & \multirow{7}{*}{1} \\
        %  \hline
          & Creatinine &  \\
        %  \hline
          & MISSING Lactic Dehydrogenase & \\
        %  \hline 
          & Total CO2 venous blood gas analysis &  \\
          & Magnesium &  \\
          & Gamma glutamyltransferase &  \\
          & Alanine transaminase &  \\
         \hline
         \multirow{2}{*}{8} & ctO2 arterial blood gas analysis & \multirow{2}{*}{0.999} \\
          & HCO3 venous blood gas analysis & \\
         \hline
         10 & Relationship Patient Normal & 0.786 \\
         \hline
         11 & MISSING Arteiral Fio2 & 0.595 \\
         \hline
         12 & Base excess venous blood gas analysis & 0.578 \\
         \hline
         13 & pO2 venous blood gas analysis & 0.449 \\
         \hline
         14 & MISSING International normalized ratio INR & 0.435 \\
         \hline
         15 & Mean platelet volume & 0.366 \\
         \hline
         16 & Metapneumovirus not detected & 0.308 \\
         \hline
         17 & Proteina C reativa mg dL & 0.235 \\
         \hline
         18 & Sodium & 0.212\\
         \hline
         19 & Phosphor & 0.164 \\
         \hline
         20 & Urine Density & 0.085 \\
         \hline
         21 & Respiratory Syncytial Virus detected & 0.068 \\
         \hline
         22 & MISSING Mean platelet volume & 0.056 \\
         \hline
         23 & MISSING Ferritin & 0.054 \\
         \hline
         24 & pH venous blood gas analysis & 0.021 \\
         \hline
         25 & Strepto A positive & 0.018 \\
         \hline
         26 & Inf A H1N1 2009 detected & 0.016 \\
         \hline
         27 & Influenza A rapid test positive & 0.014 \\
         \hline
         \multirow{2}{*}{28} & MISSING Albumin & \multirow{2}{*}{0.012} \\
          & Coronavirus HKU1 detected & \\
         \hline
         30 & MISSING Magnesium & 0.008 \\
         \hline
         31 & Aspartate transaminase & 0.004 \\
         \hline
         \multirow{5}{*}{32} & Urine Ketone Bodies absent & \multirow{5}{*}{0.001} \\
          & Red blood cell distribution width RDW & \\
          & Influenza A detected & \\
          & Urine Esterase absent & \\
          & Urine Protein nan & \\
          \hline
    \end{tabular}
    \end{minipage}}
    \end{minipage}%
    \hspace{1cm}
    \begin{minipage}{.45\linewidth}
        \caption[Caption for LOF]{Ranks of the features based on the times being predicted as direct causes of \textbf{Patient addmited to intensive care unit} out of 1000 different runs of our propsal approach. Not mentiond features were not predicted even once, note that preprocessed dataset has 331 features.}
	    \label{Table:Covid_exam_result4}
	    \resizebox{0.48\textwidth}{!}{\begin{minipage}{\textwidth}
            \begin{tabular}{ |c| l||c| }
         \hline  
         Rank & Feature & Rate of being Predicted as a Direct Cause \\ 
         \hline
         \hline
         \multirow{9}{*}{1} & Patient age quantile & \multirow{9}{*}{1} \\
        %  \hline
          & MISSING Mean platelet volume &  \\
        %  \hline
          & Total CO2 venous blood gas analysis & \\
        %  \hline 
          & HCO3 venous blood gas analysis &  \\
          & Alanine transaminase &  \\
          & Gamma glutamyltransferase &  \\
          & Magnesium &  \\
          & MISSING Lactic Dehydrogenase & \\
          & Creatinine & \\
         \hline
         10 & pO2 venous blood gas analysis & 0.982 \\
         \hline
         11 & ctO2 arterial blood gas analysis & 0.962 \\
         \hline
         12 & pH venous blood gas analysis & 0.938 \\
         \hline
         13 & MISSING Arteiral Fio2 & 0.667\\
         \hline
         14 & MISSING International normalized ratio INR & 0.586 \\
         \hline
         15 & Red blood cell distribution width RDW & 0.503 \\
         \hline
         16 & Urine Density & 0.414 \\
         \hline
         17 & Creatine phosphokinase CPK & 0.380 \\
         \hline
         18 & Base excess venous blood gas analysis & 0.352\\
         \hline
         19 & Potassium & 0.234 \\
         \hline
         20 & Promyelocytes & 0.221 \\
         \hline
         21 & MISSING Ferritin & 0.174 \\
         \hline
         22 & Metapneumovirus not detected & 0.132 \\
         \hline
         23 & Phosphor & 0.082 \\
         \hline
         24 & Sodium & 0.036 \\
         \hline
         25 & MISSING Magnesium & 0.032 \\
         \hline
         26 & Proteina C reativa mg dL & 0.016 \\
         \hline
         27 & Aspartate transaminase & 0.015 \\
         \hline
         28 & Respiratory Syncytial Virus detected & 0.010 \\
         \hline
         29 & Relationship Patient Normal & 0.007 \\
         \hline
         \multirow{2}{*}{30} & MISSING Albumin & \multirow{2}{*}{0.006} \\
          & Arterial Lactic Acid & \\
         \hline
         \multirow{2}{*}{32} & Coronavirus HKU1 detected & \multirow{2}{*}{0.005} \\
          & Eosinophils & \\
         \hline
         34 & Inf A H1N1 2009 detected & 0.004 \\
         \hline
         \multirow{2}{*}{35} & Influenza A rapid test positive & \multirow{2}{*}{0.002} \\
          & International normalized ratio INR & \\
         \hline
         \multirow{3}{*}{37} & Urine Crystals Ausentes & \multirow{3}{*}{0.001} \\
         & Leukocytes & \\
         & Strepto A positive & \\
         \hline
    \end{tabular}
    \end{minipage}}
    \end{minipage} 
\end{table}

% \begin{table*}[!h]
%     \small
%     \caption[Caption for LOF]{Ranks of the features based on the times being predicted as direct causes of \textbf{SARS-Cov-2 exam result} out of 1000 different runs of our propsal approach. Not mentiond features were not predicted even once, note that preprocessed dataset has 331 features.}
% 	\label{Table:Covid_exam_result1}
% 	\centering
% 	\resizebox{0.6\textwidth}{!}{\begin{minipage}{\textwidth}
%     \begin{tabular}{ |c| l||c| }
%          \hline  
%          Rank & Feature & Rate of being Predicted as a Direct Cause \\ 
%          \hline
%          \hline
%          \multirow{4}{*}{1} & Patient age quantile & \multirow{4}{*}{1} \\
%         %  \hline
%           & Arterial Lactic Acid &  \\
%         %  \hline
%           & Promyelocytes & \\
%         %  \hline 
%           & Base excess venous blood gas analysis &  \\
%          \hline
%          5 & pH venous blood gas analysis & 0.999 \\
%          \hline
%          6 & MISSING Mean platelet volume & 0.992 \\
%          \hline
%          7 & MISSING Lactic Dehydrogenase & 0.966 \\
%          \hline
%          8 & Segmented & 0.934 \\
%          \hline
%          9 & Myelocytes & 0.904 \\
%          \hline
%          10 & Eosinophils & 0.794 \\
%          \hline
%          11 & Leukocytes & 0.784 \\
%          \hline
%          12 & Total CO2 arterial blood gas analysis & 0.450 \\
%          \hline
%          13 & Potassium & 0.340 \\
%          \hline
%          14 & MISSING International normalized ratio INR & 0.289\\
%          \hline
%          15 & Metapneumovirus not detected & 0.234 \\
%          \hline
%          16 & Arteiral Fio2 & 0.092 \\
%          \hline
%          17 & HCO3 arterial blood gas analysis. & 0.046 \\
%          \hline
%          18 & Creatinine & 0.035 \\
%          \hline
%          19 & MISSING.Magnesium & 0.034 \\
%          \hline
%          20 & pO2 arterial blood gas analysis & 0.031 \\
%          \hline
%          21 & MISSING Arteiral Fio2 & 0.024 \\
%          \hline
%          22 & Direct Bilirubin & 0.016 \\
%          \hline
%          \multirow{2}{*}{23} & MISSING Ferritin & \multirow{2}{*}{0.014} \\
%           & Respiratory Syncytial Virus detected & \\
%           \hline
%           \multirow{2}{*}{25} & MISSING Albumin & \multirow{2}{*}{0.010} \\
%           & Creatine phosphokinase CPK & \\
%          \hline
%          27 & Strepto A positive & 0.008 \\
%          \hline
%          \multirow{4}{*}{28} & Neutrophils & \multirow{4}{*}{0.004} \\
%           & Red blood cell distribution width RDW &  \\
%          & Coronavirus HKU1 detected &  \\
%          & Influenza A rapid test positive &  \\
%          \hline
%          32 & Hb saturation venous blood gas analysis & 0.002 \\
%          \hline
%          \multirow{5}{*}{33} & Urine pH & \multirow{5}{*}{0.001} \\
%          & Inf A H1N1 2009 detected & \\
%          & MISSING Serum Glucose & \\
%          & Aspartate transaminase & \\
%          & Urine Esterase nan & \\
%          \hline
%     \end{tabular}
%     \end{minipage}}
% \end{table*}

% \begin{table*}[!t]
%     \small
%     \caption[Caption for LOF]{Ranks of the features based on the times being predicted as direct causes of \textbf{Patient addmited to regular ward} out of 1000 different runs of our propsal approach. Not mentiond features were not predicted even once, note that preprocessed dataset has 331 features.}
% 	\label{Table:Covid_exam_result2}
% 	\centering
% 	\resizebox{0.6\textwidth}{!}{\begin{minipage}{\textwidth}
%     \begin{tabular}{ |c| l||c| }
%          \hline  
%          Rank & Feature & Rate of being Predicted as a Direct Cause \\ 
%          \hline
%          \hline
%          \multirow{4}{*}{1} & Patient age quantile & \multirow{4}{*}{1} \\
%         %  \hline
%           & HCO3 venous blood gas analysis &  \\
%         %  \hline
%           & Total CO2 venous blood gas analysis & \\
%         %  \hline 
%           & Gamma glutamyltransferase &  \\
%          \hline
%          5 & MISSING Lactic Dehydrogenase & 0.987 \\
%          \hline
%          6 & Alanine transaminase & 0.845 \\
%          \hline
%          7 & MISSING International normalized ratio INR & 0.804 \\
%          \hline
%          8 & Serum Glucose & 0.652 \\
%          \hline
%          9 & pH venous blood gas analysis & 0.631 \\
%          \hline
%          10 & Base.excess venous blood gas analysis & 0.341 \\
%          \hline
%          11 & MISSING Arteiral Fio2 & 0.334 \\
%          \hline
%          12 & Urine Density & 0.334 \\
%          \hline
%          13 & Magnesium & 0.323 \\
%          \hline
%          14 & Metapneumovirus not detected & 0.261\\
%          \hline
%          15 & MISSING Mean platelet volume & 0.118 \\
%          \hline
%          16 & Creatine phosphokinase CPK & 0.086 \\
%          \hline
%          17 & Creatinine & 0.058 \\
%          \hline
%          18 & International normalized ratio INR & 0.049 \\
%          \hline
%          19 & MISSING Ferritin & 0.046 \\
%          \hline
%          20 & Urea & 0.044 \\
%          \hline
%          21 & Respiratory Syncytial Virus detected & 0.032 \\
%          \hline
%          22 & MISSING Magnesium & 0.021 \\
%          \hline
%          23 & MISSING Albumin & 0.018 \\
%          \hline
%          24 & MISSING Potassium & 0.016 \\
%          \hline
%          25 & Inf A H1N1 2009 detected & 0.014 \\
%          \hline
%          26 & Coronavirus HKU1 detected & 0.010 \\
%          \hline
%          27 & Strepto A positive & 0.008 \\
%          \hline
%          28 & Influenza A rapid test positive & 0.007 \\
%          \hline
%          \multirow{2}{*}{29} & MISSING Sodium & \multirow{2}{*}{0.002} \\
%           & Urine Protein nan & \\
%          \hline
%          \multirow{3}{*}{31} & ctO2 arterial blood gas analysis & \multirow{3}{*}{0.001} \\
%           & Influenza A detected & \\
%           & Influenza B detected & \\
%          \hline
%     \end{tabular}
%     \end{minipage}}
% \end{table*}

% \begin{table*}[!h]
%     \small
%     \caption[Caption for LOF]{Ranks of the features based on the times being predicted as direct causes of \textbf{Patient addmited to semi-intensive unit} out of 1000 different runs of our propsal approach. Not mentiond features were not predicted even once, note that preprocessed dataset has 331 features.}
% 	\label{Table:Covid_exam_result3}
% 	\centering
%     \begin{tabular}{ |c| l||c| }
%          \hline  
%          Rank & Feature & Rate of being Predicted as a Direct Cause \\ 
%          \hline
%          \hline
%          \multirow{7}{*}{1} & Patient age quantile & \multirow{7}{*}{1} \\
%         %  \hline
%           & Creatinine &  \\
%         %  \hline
%           & MISSING Lactic Dehydrogenase & \\
%         %  \hline 
%           & Total CO2 venous blood gas analysis &  \\
%           & Magnesium &  \\
%           & Gamma glutamyltransferase &  \\
%           & Alanine transaminase &  \\
%          \hline
%          \multirow{2}{*}{8} & ctO2 arterial blood gas analysis & \multirow{2}{*}{0.999} \\
%           & HCO3 venous blood gas analysis & \\
%          \hline
%          10 & Relationship Patient Normal & 0.786 \\
%          \hline
%          11 & MISSING Arteiral Fio2 & 0.595 \\
%          \hline
%          12 & Base excess venous blood gas analysis & 0.578 \\
%          \hline
%          13 & pO2 venous blood gas analysis & 0.449 \\
%          \hline
%          14 & MISSING International normalized ratio INR & 0.435 \\
%          \hline
%          15 & Mean platelet volume & 0.366 \\
%          \hline
%          16 & Metapneumovirus not detected & 0.308 \\
%          \hline
%          17 & Proteina C reativa mg dL & 0.235 \\
%          \hline
%          18 & Sodium & 0.212\\
%          \hline
%          19 & Phosphor & 0.164 \\
%          \hline
%          20 & Urine Density & 0.085 \\
%          \hline
%          21 & Respiratory Syncytial Virus detected & 0.068 \\
%          \hline
%          22 & MISSING Mean platelet volume & 0.056 \\
%          \hline
%          23 & MISSING Ferritin & 0.054 \\
%          \hline
%          24 & pH venous blood gas analysis & 0.021 \\
%          \hline
%          25 & Strepto A positive & 0.018 \\
%          \hline
%          26 & Inf A H1N1 2009 detected & 0.016 \\
%          \hline
%          27 & Influenza A rapid test positive & 0.014 \\
%          \hline
%          \multirow{2}{*}{28} & MISSING Albumin & \multirow{2}{*}{0.012} \\
%           & Coronavirus HKU1 detected & \\
%          \hline
%          30 & MISSING Magnesium & 0.008 \\
%          \hline
%          31 & Aspartate transaminase & 0.004 \\
%          \hline
%          \multirow{5}{*}{32} & Urine Ketone Bodies absent & \multirow{5}{*}{0.001} \\
%           & Red blood cell distribution width RDW & \\
%           & Influenza A detected & \\
%           & Urine Esterase absent & \\
%           & Urine Protein nan & \\
%           \hline
%     \end{tabular}
% \end{table*}


% \begin{table*}[!h]
%     \small
%     \caption[Caption for LOF]{Ranks of the features based on the times being predicted as direct causes of \textbf{Patient addmited to intensive care unit} out of 1000 different runs of our propsal approach. Not mentiond features were not predicted even once, note that preprocessed dataset has 331 features.}
% 	\label{Table:Covid_exam_result4}
% 	\centering
%     \begin{tabular}{ |c| l||c| }
%          \hline  
%          Rank & Feature & Rate of being Predicted as a Direct Cause \\ 
%          \hline
%          \hline
%          \multirow{9}{*}{1} & Patient age quantile & \multirow{9}{*}{1} \\
%         %  \hline
%           & MISSING Mean platelet volume &  \\
%         %  \hline
%           & Total CO2 venous blood gas analysis & \\
%         %  \hline 
%           & HCO3 venous blood gas analysis &  \\
%           & Alanine transaminase &  \\
%           & Gamma glutamyltransferase &  \\
%           & Magnesium &  \\
%           & MISSING Lactic Dehydrogenase & \\
%           & Creatinine & \\
%          \hline
%          10 & pO2 venous blood gas analysis & 0.982 \\
%          \hline
%          11 & ctO2 arterial blood gas analysis & 0.962 \\
%          \hline
%          12 & pH venous blood gas analysis & 0.938 \\
%          \hline
%          13 & MISSING Arteiral Fio2 & 0.667\\
%          \hline
%          14 & MISSING International normalized ratio INR & 0.586 \\
%          \hline
%          15 & Red blood cell distribution width RDW & 0.503 \\
%          \hline
%          16 & Urine Density & 0.414 \\
%          \hline
%          17 & Creatine phosphokinase CPK & 0.380 \\
%          \hline
%          18 & Base excess venous blood gas analysis & 0.352\\
%          \hline
%          19 & Potassium & 0.234 \\
%          \hline
%          20 & Promyelocytes & 0.221 \\
%          \hline
%          21 & MISSING Ferritin & 0.174 \\
%          \hline
%          22 & Metapneumovirus not detected & 0.132 \\
%          \hline
%          23 & Phosphor & 0.082 \\
%          \hline
%          24 & Sodium & 0.036 \\
%          \hline
%          25 & MISSING Magnesium & 0.032 \\
%          \hline
%          26 & Proteina C reativa mg dL & 0.016 \\
%          \hline
%          27 & Aspartate transaminase & 0.015 \\
%          \hline
%          28 & Respiratory Syncytial Virus detected & 0.010 \\
%          \hline
%          29 & Relationship Patient Normal & 0.007 \\
%          \hline
%          \multirow{2}{*}{30} & MISSING Albumin & \multirow{2}{*}{0.006} \\
%           & Arterial Lactic Acid & \\
%          \hline
%          \multirow{2}{*}{32} & Coronavirus HKU1 detected & \multirow{2}{*}{0.005} \\
%           & Eosinophils & \\
%          \hline
%          34 & Inf A H1N1 2009 detected & 0.004 \\
%          \hline
%          \multirow{2}{*}{35} & Influenza A rapid test positive & \multirow{2}{*}{0.002} \\
%           & International normalized ratio INR & \\
%          \hline
%          \multirow{3}{*}{37} & Urine Crystals Ausentes & \multirow{3}{*}{0.001} \\
%          & Leukocytes & \\
%          & Strepto A positive & \\
%          \hline
%     \end{tabular}
% \end{table*}

==> TMLR 2022_ Causal Feature Selection via Orthogonal Search 2/discussion.tex <==
\section{Discussion}
\label{sec:conclusions}
%Causal structure discovery is challenging but of high importance for many fields, especially in the presence of nonlinear relationships. 
A recent empirical evaluation of different causal discovery methods highlighted the desirability of more efficient search algorithms \citep{heinze2018causal}. In the present work, we provide identifiability results for the set of direct causal parents, including the case of partially nonlinear cyclic models, as well as a highly efficient algorithm that scales well w.r.t. the number of {variables} and exhibits state-of-the-art performance across extensive experiments. Our approach builds on the Double ML method \cite{doubleml2016} \correctedbis{and properties of conditional covariance estimands, which can leverage Lasso predictors to obtain consistent estimators in high dimensional settings \cite{smucler2019unifyin}. Theoretical properties of such approaches \cite[Section 2]{smucler2019unifyin}, such as \textit{rate double robustness}, which accommodates non-strict (approximate) sparsity assumptions, as well as model double robustness, which allows some degree of model misspecification, may explain the empirically observed performance of our approach.}  % ; however, we show it can be applied to different underlying causal structures, which is the key for the purpose of search, as this structure is not always known in advance. 
Whilst not amounting to full causal graph discovery, identification of causal parents is of major interest in real-world applications, e.g., when assaying the causal influence of genes on the phenotype. A natural direction worth exploring is to extend this approach for discovering direct causal parents in the case when nonlinear relationships exist between the output variable and its direct causal parents.

\subsubsection*{Acknowledgements}

This work was supported by the German Federal Ministry of Education and Research (BMBF): T\"ubingen AI Center, FKZ: 01IS18039B.


==> TMLR 2022_ Causal Feature Selection via Orthogonal Search 2/experiments.tex <==
\section{Experiments}
\label{sec:experiments}

\begin{figure*}[h]
    \centering
    \makebox[0.6\paperwidth]{%
    \begin{tikzpicture}[ampersand replacement=\&]
        \matrix (fig) [matrix of nodes,row sep=-1.1em, column sep=-3em]{ 
            \begin{subfigure}{0.375\textwidth}
                \centering
                \resizebox{\linewidth}{!}{
                    \begin{tikzpicture}
                        \node (img)  {\includegraphics[width=0.4\textwidth]{img/new/pointplots_version1/sparsity_lasso/accuracy/n20observation_num500nonlinear_probability0alpha05beta15theta05noise_sigma01.pdf}};
                        \node[below=of img, node distance=0cm, yshift=1.2cm, font=\color{black}] {\scalebox{0.35}{Sparsity}};
                        \node[left=of img, node distance=0cm, rotate=90, anchor=center, yshift=-1cm, font=\color{black}] {\scalebox{0.35}{Accuracy}};
                    \end{tikzpicture}
                } 
                \vspace{-0.9cm}
                \caption{$p_n = 0$, $\sigma^2 = 0.1$} 
                \label{fig:subfig1}
            \end{subfigure}
        \&
             \begin{subfigure}{0.375\textwidth}
                \centering
                \resizebox{\linewidth}{!}{
                    \begin{tikzpicture}
                        \node (img)  {\includegraphics[width=0.4\textwidth]{img/new/pointplots_version1/sparsity_lasso/accuracy/n20observation_num500nonlinear_probability0alpha05beta15theta05noise_sigma05.pdf}};
                        \node[below=of img, node distance=0cm, yshift=1.2cm, font=\color{black}] {\scalebox{0.35}{Sparsity}};
                        \node[left=of img, node distance=0cm, rotate=90, anchor=center, yshift=-1cm, font=\color{black}] {\scalebox{0.35}{Accuracy}};
                    \end{tikzpicture}
                } 
                \vspace{-0.9cm}
                \caption{$p_n = 0$, $\sigma^2 = 0.5$} 
                \label{fig:subfig2}
            \end{subfigure}
        \&
             \begin{subfigure}{0.375\textwidth}
                \centering
                \resizebox{\linewidth}{!}{
                    \begin{tikzpicture}
                        \node (img)  {\includegraphics[width=0.4\textwidth]{img/new/pointplots_version1/sparsity_lasso/accuracy/n20observation_num500nonlinear_probability0alpha05beta15theta05noise_sigma1.pdf}};
                        \node[below=of img, node distance=0cm, yshift=1.2cm, font=\color{black}] {\scalebox{0.35}{Sparsity}};
                        \node[left=of img, node distance=0cm, rotate=90, anchor=center, yshift=-1cm, font=\color{black}] {\scalebox{0.35}{Accuracy}};
                    \end{tikzpicture}
                } 
                \vspace{-0.9cm}
                \caption{$p_n = 0$, $\sigma^2 = 1.0$} 
                \label{fig:subfig3}
            \end{subfigure}
        \&
        \\
             \begin{subfigure}{0.375\textwidth}
                \centering
                \resizebox{\linewidth}{!}{
                    \begin{tikzpicture}
                        \node (img)  {\includegraphics[width=0.4\textwidth]{img/new/pointplots_version1/sparsity_lasso/accuracy/n20observation_num500nonlinear_probability05alpha05beta15theta05noise_sigma01.pdf}};
                        \node[below=of img, node distance=0cm, yshift=1.2cm, font=\color{black}] { \scalebox{0.35}{Sparsity}};
                        \node[left=of img, node distance=0cm, rotate=90, anchor=center, yshift=-1cm, font=\color{black}] { \scalebox{0.35}{Accuracy}};
                    \end{tikzpicture}
                } 
                \vspace{-0.9cm}
                \caption{$p_n = 0.5$, $\sigma^2 = 0.1$} 
                \label{fig:subfig4}
            \end{subfigure}
        \&
            \begin{subfigure}{0.375\textwidth}
                \centering
                \resizebox{\linewidth}{!}{
                    \begin{tikzpicture}
                        \node (img)  {\includegraphics[width=0.4\textwidth]{img/new/pointplots_version1/sparsity_lasso/accuracy/n20observation_num500nonlinear_probability05alpha05beta15theta05noise_sigma05.pdf}};
                        \node[below=of img, node distance=0cm, yshift=1.2cm, font=\color{black}] {\scalebox{0.35}{ Sparsity}};
                        \node[left=of img, node distance=0cm, rotate=90, anchor=center, yshift=-1cm, font=\color{black}] {\scalebox{0.35}{ Accuracy}};
                    \end{tikzpicture}
                } 
                \vspace{-0.9cm}
                \caption{$p_n = 0.5$, $\sigma^2 = 0.5$} 
                \label{fig:subfig5}
            \end{subfigure}
        \&
            \begin{subfigure}{0.375\textwidth}
                \centering
                \resizebox{\linewidth}{!}{
                    \begin{tikzpicture}
                        \node (img)  {\includegraphics[width=0.4\textwidth]{img/new/pointplots_version1/sparsity_lasso/accuracy/n20observation_num500nonlinear_probability05alpha05beta15theta05noise_sigma1.pdf}};
                        \node[below=of img, node distance=0cm, yshift=1.2cm, font=\color{black}] {\scalebox{0.35}{ Sparsity}};
                        \node[left=of img, node distance=0cm, rotate=90, anchor=center, yshift=-1cm, font=\color{black}] {\scalebox{0.35}{ Accuracy}};
                    \end{tikzpicture}
                } 
                \vspace{-0.9cm}
                \caption{$p_n = 0.5$, $\sigma^2 = 1.0$} 
                \label{fig:subfig6}
            \end{subfigure}
        \\
        };
        \draw[-latex] ([xshift=3mm]fig-1-1.west)  -- ([xshift=3mm]fig-2-1.west) node[midway,below,sloped]{nonlinearity};
        \draw[-latex] ([yshift=-2mm]fig-1-1.north)  -- ([yshift=-2mm]fig-1-3.north) node[midway,above]{noise level};
    \end{tikzpicture}}
    \vspace{-0.3cm}
    \caption{Overall performance for a single random DAG with 100 simulations for each setting, having 20 nodes and 500 observations. %Compared to other methods, our approach is stable \textit{w.r.t}. noise level, sparsity and even partially non-linear relationships, significantly outperforming the majority of baselines.%\Stefan{If we need to save space we can make one row with 4 plots: We show the current plots a, d, e and f in one row. Plots b and c) get deleted. } 
    }
    \label{fig:exp_overall}
\end{figure*}

%In this section, we perform extensive empirical evaluation for our method. 



\subsection{Experimental Setup}
\label{sec:exp_setup}

% \begin{wrapfigure}{r}{0.4\textwidth}
% \centering
%     \includegraphics[scale=0.17]{img/new/real_data/pnas2.pdf}
%     \vspace{-2mm}
%     \caption{Detection rate of causal links on the real world dataset \citep{scheetz2006regulation} over 100 single runs for the CORTH Algorithm. Out of 100 genes, only nodes that at least were predicted once as direct causes are included in this figure.}
%     \label{fig:pnas}
%     \vspace{-4mm}
% \end{wrapfigure}
% \vspace{-3mm}

\corrected{To showcase performance of our algorithm, we conducted two sets of experiments: i) Comparison with causal structure learning methods (Casual and Markov Blanket discovery) using data consisted of DAGs with high number of observations-to-number of variables ratio ($n \gg d$) which is applicable to causal structure learning methods. Markov Blanket discovery methods are included since under NFD, faithfulness, and no-hidden-confounders assumptions, Markov Blanket of the target variable corresponds to the direct parents. Note that, faithfulness and no-hidden-confounders assumptions are not necessary for our method. These experiments are discussed in details in~\Cref{sec:exp_causal Structure learning} ii) Comparison with inference by regression methods using data consisted of DAGs with high number of observations-to-number of variables ratio ($n \approx d$ and $n \ll d$) to illustrate performance in high-dimensional regimes. This part is explained thoroughly in~\Cref{sec:exp_regression}}

\subsubsection{\corrected{Causal Structure Learning}} \label{sec:exp_causal Structure learning}

 For every combination of number of nodes (\#nodes), connectivity $(p_s)$, noise level $(\sigma^2)$, number of observations $(n)$,  and non-linear probability $(p_n)$ (see~\Cref{tab:experiment_setup}),  100 examples (DAGs) are generated and stored as csv files (altogether 72.000 DAGs are simulated, comprising a dataset of overall $>$10GB). For each DAG, $n$ samples are generated.  We provide more details about the parameters (\#nodes, $p_s$, $p_n$ and $n$) and data generation  process in~\Cref{appendix:data_gen_causal}. For future benchmarking, the generated files with the code will be made available later. 


\corrected{The baselines we compare our method against are categorized in two groups which are suitable for observational data: i) Causal Structure Learning methods:} \textsc{LiNGAM} \citep{shimizu2006linear}, order - independent \textsc{PC} \citep{JMLR:v15:colombo14a}, rankPC,  %FCI\footnote{FCI and RankFCI did not finish in reasonable times for lots of cases out of 100 for each setting, that is the reason they are not included in the tables.}, rankFCI\footnotemark[\value{footnote}],  
MMHC~\citep{mmhc}, GES~\citep{ges}, rankGES, ARGES (adaptively restricted GES~\citep{arges}), rankARGES, FCI+~\citep{fciplus}, PCI~\citep{shah2020hardness} and Lasso\footnote{None-zero coefficients are reported.}~\citep{tibshirani1996regression}.  \corrected{ii) Markov Blanket discovery methods: Grow-Shrink (GS~\citep{margaritis1999bayesian}), Incremental Association Markov Blanket (IAMB~\citep{tsamardinos2003algorithms}), Max-Min Parents \& Children (MMPC~\citep{tsamardinos2003time}),  FastIAMB~\citep{yaramakala2005speculative}. and IAMB with FDR Correction~\citep{pena2008learning}.} The "CompareCausalNetworks"\footnote{ \url{https://cran.r-project.org/web/packages/CompareCausalNetworks/index.html}} \corrected{and "bnlearn: Bayesian Network Structure Learning, Parameter Learning and Inference"}\footnote{\url{https://cran.r-project.org/web/packages/bnlearn/}} R Packages are used to run most of the baselines methods. We use 10-fold cross-validation to choose the parameters of all approaches. As direction of the possible causes in the defined setting is determined, the non-directional edges inferred by some baselines, e.g., \textsc{PC} are evaluated as direct causes of the target variable.


\subsubsection{\corrected{Inference by Regression}} \label{sec:exp_regression}

\corrected{Similar to the previous section, for every combination of parameters, 50 examples are generated and stored, which means 15000 DAGs overall. Details are provided in~\Cref{appendix:data_gen_reg}}
\corrected{
We compare our algorithm to methods for inference in regression models: Standard Regression, Lasso with exact post-selection inference~\citep{lee2016exact}, Debiased Lasso~\citep{javanmard2015biasing}, Forward Stepwise Regression for active variables~\citep{loftus2014significance,tibshirani2016exact}, Forward Stepwise Regression for all variables~\citep{loftus2014significance,tibshirani2016exact}, LARS for active variables~\citep{efron2004least,tibshirani2016exact}, and LARS for all variables~\citep{efron2004least,tibshirani2016exact}. "selectiveInference: Tools for Post-Selection Inference"  R Package \footnote{https://cran.r-project.org/web/packages/selectiveInference/} is leveraged to run most of these baselines. We used cross-validation to choose hyperparameters and confidence level for hypothesis testing considered is $90\%$. 
}


\begin{figure*}[!t]
    \centering
    \begin{tikzpicture}    
        \matrix (fig) [matrix of nodes, row sep=-1.1em, column sep=-3em]{ 
            \begin{subfigure}{0.38\textwidth}
                \centering
                \resizebox{\linewidth}{!}{
                    \begin{tikzpicture}
                        \node (img)  {\includegraphics[width=0.32\textwidth]{img/new/parameter_estimations_version1/parentVSnonparent_lasso/sparsity03n20observation_num20000nonlinear_probability03alpha05beta15theta05noise_sigma03.pdf}};
                        \node[below=of img, node distance=0cm, yshift=1.22cm, font=\color{black}] {  \scalebox{0.3}{$\hat{\theta}$} };
                    \end{tikzpicture}
                } 
                \vspace{-0.9cm}
                \caption{$p_n = 0.3$, $\sigma^2 = 0.3$} 
                \label{fig:estimation_subfig1}
            \end{subfigure}
        &
            \begin{subfigure}{0.38\textwidth}
                \centering
                \resizebox{\linewidth}{!}{
                    \begin{tikzpicture}
                        \node (img)  {\includegraphics[width=0.32\textwidth]{img/new/parameter_estimations_version1/parentVSnonparent_lasso/sparsity03n20observation_num20000nonlinear_probability03alpha05beta15theta05noise_sigma05.pdf}};
                        \node[below=of img, node distance=0cm, yshift=1.22cm, font=\color{black}] {  \scalebox{0.3}{$\hat{\theta}$} };
                    \end{tikzpicture}
                } 
                \vspace{-0.9cm}
                \caption{$p_n = 0.3$, $\sigma^2 = 0.5$} 
                \label{fig:estimation_subfig2}
            \end{subfigure}
        &
             \begin{subfigure}{0.38\textwidth}
                \centering
                \resizebox{\linewidth}{!}{
                    \begin{tikzpicture}
                        \node (img)  {\includegraphics[width=0.32\textwidth]{img/new/parameter_estimations_version1/parentVSnonparent_lasso/sparsity03n20observation_num20000nonlinear_probability03alpha05beta15theta05noise_sigma1.pdf}};
                        \node[below=of img, node distance=0cm, yshift=1.22cm, font=\color{black}] {  \scalebox{0.3}{$\hat{\theta}$} };
                    \end{tikzpicture}
                } 
                \vspace{-0.9cm}
                \caption{$p_n = 0.3$, $\sigma^2 = 1.0$} 
                \label{fig:estimation_subfig3}
            \end{subfigure}
        \\
        % &
        %      \begin{subfigure}{0.65\columnwidth}
        %         \centering
        %         \resizebox{\linewidth}{!}{
        %             \begin{tikzpicture}
        %                 \node (img)  {\includegraphics[0.3\columnwidth]{img/new/parameter_estimations_version1/parentVSnonparent_lasso/sparsity03n20observation_num20000nonlinear_probability1alpha05beta15theta05noise_sigma1.pdf}};
        %                 \node[below=of img, node distance=0cm, yshift=1cm, font=\color{black}] { \[ \scalebox{10}{$\hat{\theta}$} \]};
        %             \end{tikzpicture}
        %         } 
        %         \caption{prob. nonlinear 1, noise level 1} 
        %         \label{fig:estimation_subfig6}
        %     \end{subfigure}
        % \\
        };
        % \draw[-latex] ([xshift=-1mm]fig-1-1.west)  -- ([xshift=-1mm]fig-2-1.west) node[midway,below,sloped]{nonlinearity};
        \draw[-latex] ([yshift=-2mm]fig-1-1.north)  -- ([yshift=-2mm]fig-1-3.north) node[midway,above]{noise level};
    \end{tikzpicture}
    \vspace{-0.3cm}
    \caption{Distribution of the estimated $\theta$ values for the true and false causal parents in 100 simulations of the graph with 20 nodes,  20000 observations and 0.3 as connectivity. The vertical lines indicate the ground truth values for the linear coefficients corresponding to  causal parents. 
    % Plots for all other estimation settings are in the Appendix~\ref{appendix:estimations}. %We observe that in all settings, the parameter estimation works reliably and well. 
    } 
    \label{fig:estimation}
\end{figure*}

\paragraph{Regression Technique and Hyper-parameters:} We use Lasso as the estimator of conditional expectation for our method because the variance bound for $\chi_j$ with Lasso type estimator of conditional expectation is provided in~\eqref{eq:var_bound}.  Further, using more splits than $2$ splits in the experiment relatively increases the performance of parameter estimation. See~\Cref{fig:estimation} for parameter estimations.

\corrected{\paragraph{Evaluation:} Recall, Fall-out, Critical Success Index, Accuracy, F1 Score, and Matthews correlation coefficient \citep{matthews1975comparison} are considered as metrics for the evaluation. These metrics are described in  Appendix~\ref{appendix:metrics}.}

% \begin{table}[bh]
% \begin{minipage}[b]{0.45\linewidth}\centering
%   \scriptsize  
%     \vspace{-0.3cm}
% 	\centering
	
% 	\begin{tabular}{ l r  rr  rr  r} %@{\extracolsep{\fill}}
% 	  \toprule
% 		& \multicolumn{6}{c}{Number of Nodes} \\
% 		\hline
% 		\multirow{2}{*}{Method} & %\multicolumn{3}{c|}{5} &
% 		\multicolumn{2}{c}{10} & \multicolumn{2}{c}{20} & \multicolumn{2}{c}{50} \\
% 		\multicolumn{1}{c}{}  & ACC & F1 & ACC & F1 & ACC & F1 \\
% 		\midrule
% 		GES & 0.85 & 0.78 & 0.74 & 0.53 & 0.70 & 0.32 \\
% 		rankGES & 0.85 & 0.75 & 0.74 & 0.51 & 0.70 & 0.32 \\
% 		%\hline
% 		%\hline
% 		ARGES & 0.80 & 0.58 & 0.75 & 0.52 & 0.71 & 0.22 \\
% 		rankARGES & 0.79 & 0.57 & 0.75 & 0.51 & 0.71 & 0.22 \\
% 		%\hline
% 		%\hline
% 	    FCI+ & 0.87  & 0.81 & 0.83 & 0.70 & 0.77  & 0.49 \\
% 		%\hline
% 		%\hline
% 		LINGAM & \textbf{0.95}  & 0.89 & 0.89 & 0.78 & 0.75  & 0.39 \\
% 		%\hline
% 		%\hline
% 		PC & 0.86  & 0.79 & 0.82 & 0.66 & 0.76  & 0.46 \\
% 		rankPC & 0.85  & 0.77 & 0.81  & 0.64 & 0.75 & 0.43 \\
% 		%\hline 
% 		%\hline 
% 		MMPC & 0.82 & 0.53 & 0.79 & 0.49 & 0.75 & 0.35 \\
% 		%\hline 
% 		%\hline
% 		MMHC  & 0.84  & 0.74 & 0.77  & 0.51 & 0.73  & 0.28 \\
% 		%\hline 
% 		%\hline
% 		GS & 0.85 & 0.60 & 0.82 & 0.58 & 0.76 & 0.39 \\
% 		%\hline 
% 		%\hline
% 		IAMB & 0.79 & 0.51 & 0.81 & 0.50 & 0.77 & 0.34 \\
% 		%\hline 
% 		%\hline
% 		FastIAMB & 0.86 & 0.61 & 0.83 & 0.59 & 0.77  & 0.41 \\
% 		%\hline 
% 		%\hline
% 		IAMB-FDR & 0.83 & 0.53 & 0.82 & 0.56 & 0.77 & 0.41\\
% 		%\hline 
% 		%\hline
% 		PCI  & 0.92  & 0.87 & 0.88  & 0.78 & 0.77  & 0.49 \\
% 		%\hline 
% 	%	\hline
% 		Lasso  & 0.91  & 0.90 & 0.90 & 0.87 & 0.77 & 0.63 \\
% 		\texttt{CORTH Features} & \textbf{0.95} & \textbf{0.93} & \textbf{0.95}  & \textbf{0.91} & \textbf{0.80}  & \textbf{0.66} \\
% 	     \bottomrule
% 		\end{tabular}
% 			\caption{Performance across all the settings for different number of nodes (10, 20 and 50). Each entry in the table is averaged over 18000 simulations. }
% 			\label{tab:results_n}
% % 			\vspace{-0.9cm}
% \end{minipage}
% \hspace{0.8cm}
% \begin{minipage}[b]{0.45\linewidth}
% \centering
% \scriptsize  
%     % \vspace{-5mm}
% 	\centering
	
% 	\begin{tabular}{ l r  rr  rr  r} %@{\extracolsep{\fill}}
% 	  \toprule
% 		& \multicolumn{6}{c}{Connectivity} \\
% 		\hline
% 		\multirow{2}{*}{Method} & %\multicolumn{3}{c|}{5} &
% 		\multicolumn{2}{c}{0.1} & \multicolumn{2}{c}{0.3} & \multicolumn{2}{c}{0.5} \\
% 		\multicolumn{1}{c}{}  & ACC & F1 & ACC & F1 & ACC & F1 \\
% 		\midrule
% 		GES & 0.96  & 0.82  & 0.81  & 0.60  & 0.65  & 0.48  \\
% 		rankGES & 0.95  & 0.79  & 0.81  & 0.58  & 0.64  & 0.47  \\
% 		%\hline
% 		%\hline
% 		ARGES & 0.96  & 0.83  & 0.80  & 0.50  & 0.61  & 0.33  \\
% 		rankARGES & 0.96  & 0.80  & 0.80  & 0.49  & 0.61  & 0.33  \\
% 		%\hline
% 		%\hline
% 		FCI+ & 0.97 & 0.85  & 0.87  & 0.71  & 0.73  & 0.63  \\
% 		%\hline
% 		%\hline
% 		LINGAM & 0.97  & 0.80  & 0.90  & 0.75  & 0.83  & 0.73  \\
% 		%\hline
% 		%\hline
% 		PC & 0.97  & 0.85  & 0.86  & 0.69 & 0.72  & 0.59 \\
% 		rankPC & 0.97  & 0.83  & 0.85 & 0.67  & 0.70  & 0.56  \\
% 		%\hline 
% 		%\hline 
% 		MMPC & 0.95 & 0.64 & 0.81 & 0.45 & 0.64 & 0.39 \\
% 		%\hline 
% 		%\hline
% 		MMHC & 0.98  & 0.87  & 0.83  & 0.56  & 0.64  & 0.40  \\
% 		%\hline 
% 		%\hline
% 		GS & 0.95 & 0.67 & 0.84 & 0.52 & 0.69 & 0.45  \\
% 		%\hline 
% 		%\hline
% 		IAMB & 0.97 & 0.74 & 0.84 & 0.52 & 0.69 & 0.45 \\
% 		%\hline 
% 		%\hline
% 		FastIAMB & 0.95 & 0.68 & 0.84 & 0.53 & 0.70 & 0.47 \\
% 		%\hline 
% 		%\hline
% 		IAMB-FDR & 0.95 & 0.63 & 0.83 & 0.49 & 0.69 & 0.45\\
% 		%\hline 
% 		%\hline
% 		PCI & 0.99  & 0.92 & 0.91 & 0.76  & 0.78  & 0.66  \\
% 		%\hline 
% 		%\hline
% 		Lasso & 0.98  & 0.92  & 0.88  & 0.81  & 0.80  & 0.78 \\
% 		\texttt{CORTH Features} & \textbf{0.99}  & \textbf{0.93}  & \textbf{0.93} & \textbf{0.86}  & \textbf{0.85} & \textbf{0.81}  \\
% 	     \bottomrule
% 		\end{tabular}
% 			\caption{Performance across all the settings for different connectivities (0.1, 0.3 and 0.5). Each single entry in the table is averaged over 24000 simulations.}
% 			\label{tab:results_s}
% % 			\vspace{-0.24cm}
% \end{minipage}
% \vspace{-0.57cm}
% \end{table}

\subsection{Results}
%\corrected{The results of the mentioned two sets of experiments are discussed below.}

\subsubsection{\corrected{Causal Structure Learning}} \label{sec:res_causal Structure learning}

Results aggregated by the number of observations (corresponding to 24000  simulations per entry in the table) are illustrated in \Cref{tab:results_o}\footnote{Please refer to~\Cref{appendix:tables} for thorough tables for all parameters.}. Our method performs better than the competing baselines in terms of accuracy and F1 score, especially for more connected structures, despite data being generated according to DAG causal structures, which, dissimilar to our method, is an essential condition for them. To provide a visual comparison, we plot the accuracy of all methods w.r.t. the connectivity parameter ($p_s$) in~\Cref{fig:exp_overall} for different values of $p_n$ and $\sigma^2$ on 1800 samples. 








It can be observed that the accuracies of the competing baselines significantly drop with increasing noise level and nonlinearity, while our method is more robust to them.
% More plots are given in~\Cref{appendix:accuracy}  and~\Cref{appendix:f1} for several other combinations of varying parameters in the simulation.
We also extensively compare all the metrics (Recall, Fall-out, Critical Success Index, Accuracy, F1 Score, and Matthews correlation coefficient) for all the methods in Appendix~\ref{appendix:tables}. According to these metrics, our approach performs better than baselines in most cases regardless of the set of parameters used for generating data. Our method shows in particular stability in performance w.r.t. the number of nodes (\Cref{Table_Number_of_Nodes}), partially non-linear relationships (\Cref{Table_Nonlinearity}), connectivity (\Cref{Table_Sparsity}), number of observations (\Cref{Table_Observation}), and noise level (\Cref{Table_Noise}). We also show the plot of parameter estimation for direct causal parents vs. non-causal parents in~\Cref{fig:estimation}. In the plots and tables, we denote our approach as \texttt{CORTH Features}.

\begin{figure}[ht]
    \begin{minipage}[b]{0.45\linewidth}
     \centering
        \vspace{0mm}
        \begin{tikzpicture}
            \node (img)  {\includegraphics[width=7cm,height=6cm]{img/new/runtime_plot/sparsity03observation_num5000nonlinear_probability0noise_sigma1.pdf}};
            \node[below=of img, node distance=0cm, xshift = 0.35cm, yshift=1cm, font=\color{black}] {\small Number of nodes};
            \node[left=of img, node distance=0cm, rotate=90, anchor=center, yshift=-0.9cm, font=\color{black}] {\small Runtime (sec)};
        \end{tikzpicture}
    
        \caption{Runtime as a function of the number of variables for 10 simulations per number of nodes. In these simulations connectivity, number of observations, nonlinaer prob., and noise level are set to 0.3, 5000, 0, and 1 respectively.}
        \label{fig:runtimes}
       \vspace{-3mm}
    \end{minipage}
\hspace{0.5cm}
    \begin{minipage}[b]{0.45\linewidth}
        \scriptsize  
        \vspace{-15mm}
    	\centering
    	
    	\begin{tabular}{ l r  rr  rr  r} %@{\extracolsep{\fill}}
    	  \toprule
    		& \multicolumn{6}{c}{Number of Observations} \\
    		\hline
    		\multirow{2}{*}{Method} & %\multicolumn{3}{c|}{5} &
    		\multicolumn{2}{c}{100} & \multicolumn{2}{c}{500} & \multicolumn{2}{c}{1000} \\
    		\multicolumn{1}{c}{}  & ACC & F1 & ACC & F1 & ACC & F1 \\
    		\midrule
    		GES & 0.80  & 0.59  & 0.81 & 0.65  & 0.81  & 0.67  \\
    		rankGES & 0.79  & 0.56  & 0.81  & 0.64  & 0.81  & 0.65  \\
    		%\hline
    		%\hline
    		ARGES & 0.78  & 0.49  & 0.80  & 0.58 & 0.80  & 0.59  \\
    		rankARGES & 0.78  & 0.47  & 0.79  & 0.57  & 0.80  & 0.58 \\
    		%\hline
    		%\hline
    		FCI+ & 0.84  & 0.67  & 0.86  & 0.75  & 0.87  & 0.78  \\
    		%\hline
    		%\hline
    		LINGAM & 0.84  & 0.65 & 0.91  & 0.74  & 0.94  & 0.88  \\
    		%\hline
    		%\hline
    		PC & 0.83  & 0.64  & 0.86  & 0.73  & 0.87  & 0.75  \\
    		rankPC & 0.82 & 0.62  & 0.85  & 0.71  & 0.85  & 0.73  \\
    		%\hline 
    		%\hline 
    	   	MMPC & 0.77 & 0.37 & 0.82 & 0.53 & 0.83 & 0.57 \\
		    %\hline 
		    %\hline
    		MMHC & 0.80  & 0.56  & 0.82  & 0.62  & 0.83  & 0.64 \\
    		%\hline 
    		%\hline
    		GS & 0.79 & 0.43 & 0.84 & 0.59 & 0.86 & 0.62  \\
    		%\hline 
    		%\hline
    		IAMB & 0.74 & 0.39 & 0.81 & 0.57 & 0.83 & 0.61 \\
		    %\hline 
		    %\hline
		    Fast-IAMB & 0.80 & 0.46 & 0.84 & 0.59 & 0.86 & 0.62 \\
		    %\hline 
		    %\hline
		    IAMB-FDR & 0.78 & 0.37 & 0.84 & 0.58 & 0.85 & 0.61 \\
		    %\hline 
		    %\hline
    	    PCI & 0.83 & 0.59  & 0.91  & 0.85 & 0.93  & 0.89  \\
    		%\hline 
    		%\hline
    		Lasso & 0.87  & \textbf{0.81}  & 0.89  & 0.85  & 0.89 & 0.85  \\
    		\texttt{CORTH Features} & \textbf{0.88} & 0.78 & \textbf{0.93}  & \textbf{0.91}  & \textbf{0.94}  & \textbf{0.92}  \\
    	     \bottomrule
    		\end{tabular}
    		\captionof{table}{Performance across all the settings for different number of observations (100, 500 and 1000). Each single entry in the table is averaged over 24000 simulations. Our method is almost state of the art in every case.}
    % 			\caption{}
    			\label{tab:results_o}
    \end{minipage}
\end{figure}


\subsubsection{\corrected{Inference by Regression}} \label{sec:res_reg}
\corrected{Analogous to previous part, results are aggregated by nonlinear probability (corresponding to 3750 simulations per entry in the table), number of observations
(3000 simulations per entry in the table), connectivity (5000 simulations per entry in the table) and beta distribution parameters are provided in~\Cref{Table_reg_Nonlinear Probability,Table_reg_Number of Observations,Table_reg_sparsity,Table_reg_alpha_beta}. Based on these results, our method suggests more robustness w.r.t. the set of parameters used for generating data and relatively better performance compared to other methods.
}


\subsection{Scaling Causal Inference to Large Graphs}
Figure \ref{fig:runtimes} shows the runtime of the method in secs as a function of the graph's size. Notice that the runtime of our algorithm in the log-log plot is roughly linear, supporting our above statement about the computational time being polynomial in $d$. As we used 5000 observations, additional overhead comes from cross-validation. 


\subsection{Real-World Data}
We also apply our algorithm to a recent COVID-19 Dataset~\citep{COVID19} where the task is to predict COVID-19 cases (confirmed using RT-PCR) amongst suspected ones. For an existing and extensive analysis of the dataset with predictive methods, we refer to \cite{schwab2020predcovid}. We apply our algorithm to discover the features which directly cause the diagnosed infection. We found that the following were the most common causes across different runs of our approach: Patient age quantile, Arterial Lactic Acid, Promyelocytes, and Base excess venous blood gas analysis. 
Lacking medical ground truth, we report these not as corroboration of our approach but rather as a potential contribution to causal discovery in this challenging problem. It is encouraging that some of these variables are consistent with other studies \cite{schwab2020predcovid}. Details on data preprocessing and more results are available in Appendix~\ref{appendix:covid}.

% \begin{wrapfigure}{r}{0.5\textwidth}
%     \centering
%     \vspace{-10mm}
%     \begin{tikzpicture}
%         \node (img)  {\includegraphics[scale=0.43]{img/new/runtime_plot/sparsity03observation_num5000nonlinear_probability0noise_sigma1.pdf}};
%         \node[below=of img, node distance=0cm, xshift = 0.35cm, yshift=1cm, font=\color{black}] {\small Number of nodes};
%         \node[left=of img, node distance=0cm, rotate=90, anchor=center, yshift=-0.9cm, font=\color{black}] {\small Runtime (sec)};
%     \end{tikzpicture}

%     \caption{Runtime as a function of the number of variables for 10 simulations per number of nodes. In these simulations connectivity, number of observations, nonlinaer prob., and noise level are set to 0.3, 5000, 0, and 1 respectively.}
%     \label{fig:runtimes}
%   \vspace{-3mm}
% \end{wrapfigure}











==> TMLR 2022_ Causal Feature Selection via Orthogonal Search 2/introduction.tex <==
\section{Introduction}

Identifying causal relationships is a profound and hard problem pervading experimental sciences such as biology \citep{sachs2005causal}, medicine \citep{castro2020causality}, earth system sciences \citep{runge2019inferring}, or robotics \citep{ahmed2020causalworld}. While randomized controlled interventional studies are considered the gold standard, they are in many cases ruled out by financial or ethical concerns \citep{pearl2009causality, spirtes2000causation}.  In order to improve the understanding of a system and help design relevant interventions, the subset of causes that have a direct effect (\textit{direct causes}/\textit{direct causal parents}) often needs to be identified based on observations only. 
\corrected{This paper assumes a structural equation model (SEM) comprising (1) a set of $d$ covariates represented by random vector $X \in \mathbb{R}^d$ whose values are determined by a uniquely solvable set of $d$ structural equations, possibly non-linear and possibly including cycles and confounding (2) a response variable $Y\in \mathbb{R}$, who is not a parent of any $X$ and whose value is determined by a linear structural equation of the form,%as described in Figure~\ref{fig:graph_description}
\begin{align} 
    Y\coloneqq \langle \theta, X\rangle + U\,,\, \mbox{ with }\theta \in \mathbb{R}^d, \label{eq:model_est}
\end{align}
where $U$ is an exogenous variable with zero mean, independent from any other exogenous variables of the SEM and $\langle\cdot,\cdot\rangle$ denotes the inner product.  Such a SEM is exemplified in  Figure~\ref{fig:graph_description}. Uniquely solvability of SEMs amounts to not having self-cycles in the causal structure, but any other arbitrary non-linear cyclic structure between covariates is allowed~\citep{bongers2021foundations}, possibly including hidden confounders, as long as there is no hidden confounder for the response variable (this would violate the assumption of independence of $U$).  Practically speaking, almost all causal discovery applications lie under the umbrella of simple SCMs~\citep{bollen1989structural, sanchez2019estimating}. Besides, the assumption of not having self-cycles is usually assumed not-limiting in the literature~\citep{lacerda2012discovering, rothenhausler2015backshift, bongers2016theoretical}.} 

In this paper, we investigate how to find the direct causes of $Y$ among a high-dimensional vector of covariates $X$. %In order for words, the causal structure of covariates ($X$) is an arbitrary member of uniquely solvable structural causal models (Simple SCMs), possibly with hidden confounders (as long as there is no hidden confounder for the response variable). 
 From our formulation, {a given entry} of {$\theta$} should be non-zero if {and only if} the variable corresponding to that particular coefficient is a direct causal parent \citep{peters2017elements}, e.g., $X_1$ and $X_2$ in Figure~\ref{fig:graph_description}. 
We restrict ourselves to the setting of \textit{linear direct causal effects} of $Y$ (LDC, as specified in Equation~\ref{eq:model_est}) and \textit{no feature descending from} $Y$ (NFD). LDC is justified as an approximation when the effects of each causal feature are weak such that the possibly non-linear effects can be linearized; NFD is justified in some applications where we can exclude any influence of $Y$ on a covariate. This is, for example, the case when $X$ are genetic factors, and $Y$ is a particular trait/phenotype. Our method, in particular, comes handy in this case due to the relatively complex non-linear cyclic structure of these genetic factors in high-dimensional regimes~\citep{yao2015prior, meinshausen2016methods, warrell2020cyclic}.

While applicable to full graph discovery rather than the simplified problem of finding causal parents, state-of-the-art methods for causal discovery often rely on strong assumptions or the availability of interventional data or have prohibitive computational costs explained in section~\ref{sec:related_work}. In addition to and despite their strong assumptions, causal discovery methods may perform worse than simple regression baselines \citep{heinze2018causal, janzing2019causal,zheng2018dags}. \correctedbis{However, estimating $\theta$ in high dimensional settings (i.e. $\#$ observations $<<d$ ) using unregularized least squares regression, will lead to identifiability problems since there can be infinitely many possible choices for $\theta$ recovered with equivalent prediction accuracy for regressing $Y$ \citep{buhlmann2011statistics}. On the other hand, when using a regularized method such as Lasso, a critical issue is the bias induced by regularization \citep{javanmard2018debiasing}. While regularized and unregularized Least Squares as well as debiased Lasso are applicable to the same problem, they have different statistical characteristics and we will explore their empirical performance in extensive experiments. }

\begin{wrapfigure}{thp}{0.4\textwidth}
% \centering
    \includegraphics[height=5.5cm]{img/CORTH_diagram.png}
    \caption{Graphical representation of Causal Feature Selection in our setting, for the case of two direct causal parents of $Y$, $X_1$ and $X_2$, out of variables $\{X_1,\cdots,X_{6} \}$, such that $Y = \theta_1X_1 + \theta_2X_2 + U$, $U$ being an independent zero-mean noise. We propose an approach to find $X_1$ and $X_2$
     under assumptions discussed in the text. An example of this setup in the real-world is finding genes which directly cause a phenotype. }
    \label{fig:graph_description}
    \vspace{-12.5mm}
\end{wrapfigure}

Double ML approaches \citep{doubleml2016} have shown promising bias compensation results in the context of high dimensional observed confounding of a single variable. In the present paper, we  use this approach to find direct causes among a large number of covariates. 
Our key contributions are:
 \begin{itemize}[noitemsep]
% \setlength\itemsep{0.001em}
    \item  We show that under the assumption that no feature of $X$ is a child of $Y$, the Double ML \citep{NeweyCherno19} principle can be applied in an iterative and parallel way to find the subset of direct causes with observational data. 
    
     \item Our approach has a computational complexity requirement polynomial (fast) time in dimension $d$.
    
    \item  Our method provides asymptotic guarantees that the set can be recovered   from observational data. Importantly, this result neither requires linear interactions among the covariates, faithfulness, nor acyclic structure. 
    
    \item Extensive experimental results demonstrate the state-of-the-art performance of our method. Our approach significantly outperforms all other methods (even though underlying data generation conditions favor them), especially in the case of non-linear interactions between covariates, despite relying only on linear projection. 
\end{itemize}


\subsection{Related work}
\label{sec:related_work}
The question of finding direct causal parents is also addressed in the literature as mediation analysis~\citep{baron1986moderator,hayes2017introduction,shrout2002mediation}. Several principled approaches have been proposed (relying, for instance, on Instrumental Variables (IVs)) \citep{angrist1995identification,angrist1996identification,bowden1990instrumental} to test for a single direct effect in the context of specific causal graphs. Extensions of the IV-based approach to generalized IVs-based approaches \citep{brito2012generalized,van2016searching} are the closest known result to discovering direct causal parents. However, no algorithm is provided in \cite{brito2012generalized}  to identify the instrumental set. Subsequently, an algorithm is provided in \cite{van2016searching}  for discovering the instrumental set in the simple setting where all the interactions are linear and the graph is acyclic. In contrast, our method allows non-linear cyclic interaction amongst the variables. 

Several other works have also tried to address the problem of discovering causal features. The authors review work on causal feature selection in \cite{guyon2007causal}. More recent papers on causal feature selection have appeared since~\citep{cawley2008causal,paul2017feature,yu2018unified}, but none of those claims to recover all the direct causal parents asymptotically or non-asymptotically as we do in our case. 
\correctedbis{There has been another line of works on inferring causal relationships from observational data based on conditional independences, such as the $\mathrm{PC}$-algorithm, which can be used for more general causal inference purposes, at the expense of extra assumptions, such as faithfulness, allowing  inference of the Markov equivalence class through testing iterative testing of d-separation statements  \citep{MasSchJan19,pearl2009causality,spirtes2000causation}.} %Classical approaches along these lines include the $\mathrm{PC}$-algorithm \citep{spirtes2000causation}, which can only reconstruct the network up to a Markov equivalence class. 
\correctedbis{In contrast, under our LDC, NFD and totally independent U assumptions, only a small subset of d-separation relationships are relevant, and further, these assumptions imply that the observed relevant conditional independences and associated d-separation are equivalent, so that a full set of faithfulness assumptions about conditioning sets besides $X_{-j}$ are not necessary.}

Another approach is to restrict the class of interactions among the covariates and the functional form of the signal-noise mixing (typically considered additive) or the distribution (e.g., non-Gaussianity) to achieve identifiability (see \citep{hoyer2009nonlinear,peters2014causal}); this includes linear approaches like $\mathrm{LiNGAM}$ \citep{shimizu2006linear} and nonlinear generalizations with additive noise \citep{Peters2011b}. For a recent review of the empirical performance of structure learning algorithms and a detailed description of causal discovery methods, we refer to \citep{heinze2018causal}. Recently, there have been several attempts at solving the problem of causal inference by exploiting the invariance of a prediction under a causal model given different experimental settings \citep{ghassami2017learning,icp2016}. The computational cost to run both algorithms is exponential in the number of variables when aiming to discover the full causal graph.

Our method mainly takes inspiration from Debiased/Double ML method \citep{doubleml2016} which utilizes the concept of orthogonalization to overcome the bias introduced due to regularization. We will discuss this in detail in the next section. Considering a specific example, the Lasso suffers from the fact that the estimated coefficients are shrunk towards zero, which is undesirable \citep{tibshirani2017sparsity}. To overcome this limitation, a debiasing approach was proposed for the Lasso in several papers \citep{javanmard2014confidence,javanmard2018debiasing,zhang2014confidence}. However, unlike our approach, Debiased Lasso methods do not recover all the non-zero coefficients of the parameter vector $\theta$ under the generic assumptions of the present work. \correctedbis{To be more specific, \citep{javanmard2018debiasing} is built upon the \Cref{eq:model_est} with the following differences to our setting: Noise $U$ is Gaussian; $X$ has independent zero-mean Gaussian rows with covariance matrix $\Sigma$ satisfying specific bounding conditions; sparsity conditions $s_0 = o(n/{(\log p)}^2)$\footnote{$p = d - 1$ is the covariate dimension.} and $\min(s_{\Omega}, s_{0}) = o(\sqrt{n}/\log p)$ where $s_0$ and $s_{\Omega}$ are sparsity levels of the true coefficients $\theta$ and the precision matrix $\Omega = \Sigma ^ {-1}$ of $X$ respectively.}

==> TMLR 2022_ Causal Feature Selection via Orthogonal Search 2/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> TMLR 2022_ Causal Feature Selection via Orthogonal Search 2/methodology.tex <==
\section{Methodology}
\label{sec:method}
Before describing the proposed method, we discuss \corrected{our general strategy as well as }Double ML and Neyman orthogonality in the next sections, which will be helpful in building the theoretical framework for our method. 
\corrected{\subsection{Reduction to a nonparametric estimation problem}\label{sec:nonpar}
According to \Cref{eq:model_est}, determining whether $X_j$ is a parent of $Y$ in our setting amounts to testing whether $\theta_j \neq 0$. Let $X_{-j}=X\setminus X_j$, this can be reduced to testing whether the following estimand vanishes:
\begin{equation}\label{eq:estimand}
\chi_{j} \triangleq \E\left[ \left(Y - \E(Y\mid X_{-j}) \right) \left(X_{j} - \E(X_{j}\mid X_{-j}) \right)\right]%=\E\left[ \left(Y - \E(Y\mid X_{-j}) \right) \left(X_{j} - \E(X_{j}\mid X_{-j}) \right)\right].
\end{equation}
Indeed,  $U$ independent of $X$ entails $Y-\E(Y\mid X_{-j})=\theta_j \left(X_j-\E(X_j\mid X_{-j})\right)+U$. This leads to
\begin{equation}\label{eq:chi}
\chi_j = \theta_j  \E\left[\left(X_j - \E(X_j\mid X_{-j})\right)^2\right]= \theta_j  \E\left[X_j\left(X_j - \E(X_j\mid X_{-j})\right)\right]\,.
\end{equation}
Under mild assumptions, testing whether $\theta_j \neq 0$ thus reduces to testing whether $\chi_j \neq 0$. \Cref{eq:estimand} shows that $\chi_j$ constitutes a \textit{non-parametric estimand}, i.e. a model-free functional of the observed data distribution. Nonparametric estimation results \citep{robins2008higher,van2011targeted,doubleml2016} make use of the  \textit{efficient influence function} of such estimand (see e.g. \citet{hines2022demystifying}) to derive valid estimates and confidence bounds, while allowing the use of data adaptive estimation strategies, such as machine learning algorithms. The resulting strategies are known as \textit{target learning} and \textit{debiased/double machine learning}, and are suitable in challenging settings such as ours when $X$ is high dimensional with possibly non-linear dependencies among components. }

\subsection{Double Machine Learning (Double ML)} \label{sec:doubleml}
\corrected{Double ML constitutes one possible way to derive efficient nonparametric estimates. We introduce it with the partial linear regression setting introduced in \citet[Example 1.1]{doubleml2016}.}
Given a fixed set of policy variables $D$ and control variables $X$ acting as common causes of $D$ and $Y$, we consider the partial regression model of~\Cref{eq:partial_regression}, 
\begin{align} 
\label{eq:partial_regression}
\begin{split} 
    Y &= D\theta_0 + g_0 (X) + U, ~~  \EE{U | X,D} =0 \\
    D &= m_0 (X) + V, ~~ \EE{V|X} = 0,
    \end{split}
\end{align}
where $Y$ is the outcome variable, $U,V$ are disturbances and $g_0,m_0: \mathbb{R}^d \rightarrow \mathbb{R}$ are (possibly non-linear) measurable functions. An unbiased estimator of the causal effect parameter $\theta_0$ can be obtained via the orthogonalization approach as in \cite{doubleml2016}, which is obtained via the use of the ``Neyman Orthogonality Condition" described below. 

\paragraph{Neyman Orthogonality Condition:} \corrected{Let $W$ denote the collection of all observed variables.} The traditional estimator of $\theta_0$ in~\Cref{eq:partial_regression} can be simply obtained by finding the zero of the empirical average of a score function ${\phi}$ such that  ${\phi}(W;\theta,g) = D^\top(Y - D\theta - g(X))$. However, the estimation of $\theta_0$ is sensitive to the bias in the estimation of the function $g$. Neyman \citep{neyman1979c} proposed an orthogonalization approach to get an estimate for $\theta_0$ that is more robust to the bias in the estimation of nuisance parameter $(m_0,g_0)$. Assume for a moment that the true nuisance parameter is $\eta_0$ (which represents $m_0$ and $g_0$ in~\Cref{eq:partial_regression}) then the orthogonalized ``score'' function $\psi$ should satisfy the property that the Gateaux derivative operator with respect to  $\eta$ vanishes when evaluated at the true parameter values:
\begin{align}
    \partial_\eta \bbE \psi(W;\theta_0, \eta_0)[\eta - \eta_0] = 0\, . \label{eq:neyman_orthogonali8ty}
\end{align}
\corrected{One way to build such a score, following \cite{doubleml2016} [eq. (2.7)], is to start from a biased score associated to maximum likelihood-like estimate. Let $\ell( {W};(\theta,\boldsymbol{\eta}))$ be the \textit{log likelihood} function or another smooth objective for which the true parameter is the unique maximizer. The true parameter then satisfies $\E \partial_\theta \ell( {W};(\theta_0,\boldsymbol{\eta}_0))=0$, suggesting to start with $\partial_\theta \ell( {W};(\theta_0,\boldsymbol{\eta_0}))$ as a (biased) score. In order to compensate the bias due to the nuisance parameters, we then subtract a linear function of the derivative of the likelihood with respect it, leading to the orthogonalized score
\begin{align*}
&\psi( {W};\theta,\boldsymbol{\eta})= \partial_\theta \ell( {W};(\theta,\boldsymbol{\eta})) - \boldsymbol{\mu} \partial_\eta \ell( {W};(\theta,\boldsymbol{\eta}))
\,.
\end{align*}
where $\boldsymbol{\mu}$ is determined by the constraint of  \Cref{eq:neyman_orthogonali8ty} (see proof of \Cref{lem:general2var_ap} in appendix).} 
The corresponding Orthogonalized  or  Double/Debiased  ML  estimator $\check{\theta}_0$  solves \corrected{a constraint of vanishing empirical average of the orthogonalized score, based on $n$-iid samples $\{W_i\}_{i=1..n}$ of the observed variables.}
 \begin{equation}
     \frac{1}{n} \sum_{i=1}^n \psi(W_i;\check\theta_0,\hat{\eta}_0) = 0,\label{eq:debiasestim}
 \end{equation}
 where $\hat{\eta}_0$ is the estimator of $\eta_0$ and $\psi$ satisfies condition in~\Cref{eq:neyman_orthogonali8ty}.  For the partially linear model discussed in~\Cref{eq:partial_regression}, the orthogonalized score function $\psi $ is,
 \begin{align}
     \psi(W;\theta,\eta) = (Y- D\theta - g(X)) (D-m(X))\,, \label{eq:orthogonal_score}
 \end{align}{}
with $\eta = (m,g)$.
\corrected{This leads to an debiased estimator satisfying
\begin{align}
     \check\theta_0 \frac{1}{n}\sum_i D_i(D_i-\check m_0(X_i))= \frac{1}{n}\sum_i (Y_i - \check g_0(X_i)) (D_i-\check m_0(X_i))\,. \label{eq:orthogonal_score2}
\end{align}
which relies on the ``double'' use of machine learning algorithm: once to learn  $\check g_0(X_i)$ and once to learn $\check m_0(X_i)$, hence the name \textit{Double ML} for such estimator.
We can further relate this approach to the design an estimator of the non-parametric estimand of previous section. 
}

\corrected{Indeed by subtracting $\check\theta_0\frac{1}{n}\sum_i \check m_0(X_i) (D_i-\check m_0(X_i))$ on both sides of \cref{eq:orthogonal_score2}, we get
\begin{align}
     \check\theta_0 \frac{1}{n}\sum_i (D_i-\check m_0(X_i))^2= \frac{1}{n}\sum_i (Y_i-\check\theta_0 \check m_0(X_i) - \check g_0(X_i)) (D_i-\check m_0(X_i))\,. \label{eq:orthogonal_score3}
\end{align}
Noticing that $\E [Y|X]=\theta_0\E [D|X]+g_0(X)=\theta_0 m_0(X)+g_0(X)$, the term $\check\theta_0 \check m_0(X_i) + \check g_0(X_i)$ in \cref{eq:orthogonal_score3} appears as an ML estimator of $\E [Y|X]$, such that we recognize on the right hand side of \Cref{eq:orthogonal_score3} a Double ML estimator of 
$
\E[(Y-\E [Y|X])(D-
\E[D|X])]
$, 
which is a special case of the non-parametric estimand $\chi_j$ defined in \Cref{eq:chi}, for the setting $X_j=D$ and $X=X_{-j}$. In practice, we directly learn an ML estimator of $\E [Y|X]$ by predicting $Y$ using $X$, relying on the double robustness of the $\chi_j$ estimands \citep{smucler2019unifyin}, as described in  \cref{subsec:test_stat}. 
}
\paragraph{From Double ML to Causal Discovery:} The distinction between policy variables and confounding variables is not always known in advance. \corrected{Fortunately, as described in \cref{sec:nonpar}, Double ML relies on estimating a non-parameteric estimand that does only depend on observational data and not on the causal model. This will allow us to exploit the same approach iteratively in the setting of causal discovery.} To this end, we consider a set of variables $X = \{ X_1, X_2, \cdots X_d \}$ which includes direct causal parents of the outcome variable $Y$ as well as other variables. We also reiterate our assumption that the relationship between the outcome variable and direct causal parents of the outcome variable is linear. The relationship among other variables can be cyclic and nonlinear. 
We now provide a general approach to scanning putative direct causes scaling ``polynomially'' in their number (see \textit{Computational Complexity} paragraph in next section), based on the application of a statistical test and Double ML estimators. We describe first the algorithm and then provide theoretical support for its performance.

\subsection{Informal Search Algorithm Description} \label{sec:algo}
Pseudo-code for our proposed method (CORTH Features) is in Algorithm~\ref{alg:double_ml_causal}. The idea is to do a one-vs-rest split for each variable in turn and estimate the link between that particular variable and the outcome variable using Double ML. To do so, we decompose~\Cref{eq:model_est} to single out a variable $D=X_k$ as policy variable and take the remaining variables $Z=X_{-k} = X\backslash X_k$ as multidimensional control variables, and run Double ML estimation assuming the partial regression model presented in~\Cref{sec:doubleml}, which now takes the form
\begin{align} 
\label{eq:searchEq}
    \begin{split} 
    Y &= D\theta_k + g_k (Z) + U, ~~  \EE{U | Z,D} =0\,, \\
    D &= m_k (Z) + V, ~~ \EE{V|Z} = 0\,.
    \end{split}
\end{align}

The step-wise description of our estimation algorithm goes as follows:

 \begin{itemize}
 %\setlength\itemsep{1mm}
 [noitemsep]
     \item[(a)] Select one of the variables $X_i$ to estimate its (hypothetical) linear causal effect $\theta$ on $Y$.
     \item[(b)] Set all of the other variables $X_{- i}$ as the set of possible confounders.
     \item[(c)] Use {the Double ML approach } to estimate the parameter $\theta$ i.e. the causal effect of $X_i$ on $Y$. 
     \item[(d)] If the variable $X_i$ is not a causal parent, the distribution of the conditional covariance $\chi_i$ (Proposition~\ref{prp:main_exp}) is a Gaussian centered around zero. We use a simple normality test for $\chi_i$ to select or discard $X_i$ as one of the direct causal parents of $Y$.  
\end{itemize}
We iteratively repeat the procedure on each of the variables until completion. Pseudo-code for the entire procedure is given below in Algorithm~\ref{alg:double_ml_causal}. \corrected{Guaranties for this approach to identify the true parents rely on the assumptions stated in \Cref{subsec:test_stat}, Equations~( \ref{eq:model1}-\ref{eq:model3}). They notably allow for hidden confounders between covariates, as long as those are not direct causes of $Y$, not descendent of $Y$. On the contrary, if $Y$ is an ancestor of any covariate, the search algorithm may fail in both directions (false positive and false negative).}

Note that~\Cref{eq:searchEq} is not necessarily a correct structural equation model to describe the true underlying causal structure. In general, for instance, when $D$ actually causes $Z$, it is non-trivial to show that the Double ML estimation of parameter $\theta_k$ will be unbiased (see~\Cref{sec:orhto_scores}).

\input{algorithm}

\paragraph{Remarks on Algorithm~\ref{alg:double_ml_causal}:} $X_i^{[k]}$ is a vector which corresponds to the samples chosen in the $k^{th}$ subsampling procedure, $X_{\backslash i}^{[k]}=(X_1^{[k]}, \dots, X_{i-1}^{[k]},X_{i+1}^{[k]},\dots,X_d^{[k]})$ for any $i\in [d]$. In general the subscript $i$ represents the estimation for the $i^{th}$ variable and super-script $k$ represents the $k^{th}$ subsampling procedure. $K$ represents the set obtained after sample splitting. $m_i^{[\backslash k]}$  are (possibly nonlinear) parametric functions fitted using $(1^{st}, \dots, {k-1}^{th}, {k+1}^{th}, \dots, K^{th})$ subsamples. 

\paragraph{Computational Complexity:} For each subset randomly selected from the data, we fit two lasso estimators.  Accelerated coordinate descent \citep{nesterov2012efficiency} can be applied to optimize the lasso objective.  To achieve $\varepsilon$ error, $\mathcal{O}\left( d\sqrt{\kappa_{\text{max}}} \log \frac{1}{\varepsilon}\right)$ number of iterations are required where $\kappa_{\text{max}}$ is the maximum of the two condition number for both the problems and each iteration requires $\mathcal{O}(nd)$ computation. Hence, the computational complexity of running our approach is only polynomial in~$d$.  


\subsection{Orthogonal Scores} \label{sec:orhto_scores}
 Now we describe the execution of our algorithm for a simple graph with 3 nodes.  Let us consider the following linear structural equation model as an example of our general formulation: 
 \begin{equation}
 %\begin{split} 
 \label{eq:sem_3_variable}
     Y  := \theta_{1}X_1 + \theta_{2} X_2 + \varepsilon_3,~ X_2 := a_{12} X_1 + \varepsilon_2 , 
      \text{ and }  X_1  := \varepsilon_1.
 %\end{split}
 \end{equation}
 
 \begin{example} \label{lem:3_variable}
Consider the system of structural equation given in~\Cref{eq:searchEq}. If $\varepsilon_1$, $\varepsilon_2$ and $\varepsilon_3$ are independent uncorrelated noise terms with zero mean, Algorithm~\ref{alg:double_ml_causal} will recover the coefficients $\theta_{1}$ and $\theta_{2}$.
 \end{example}
 
 


 
 A detailed proof is given in~\Cref{ap:proof_example1}. While the estimation of the parameter $\theta_1$ is in line with the assumed partial regression model of~\Cref{eq:sem_3_variable}, the estimation of $\theta_2$ does not follow the same. However, it can be seen from the proof that $\theta_2$  can also be estimated from the {orthogonal score} in~\Cref{eq:orthogonal_score}. 
 
  We now show that this result holds for a more general graph structure given in~\Cref{fig:general2var}, allowing for non-linear cyclic interactions among features.
 

\begin{proposition}
\label{prp:general2var}
\corrected{Assume the structural causal model of~\Cref{fig:general2var},  with (possibly non-linear and confounded) assignments between elements of $X=[X_k,X_{-k}^\top]^\top$, with $X_{-k}=[ {Z}_1^\top, {Z}_2^\top]^\top$, parameterized by $\boldsymbol{\gamma}=(\boldsymbol{\gamma}_1,\boldsymbol{\gamma}_2,\boldsymbol{\gamma}_{12})$.  %$\boldsymbol{\beta}=(\boldsymbol{\beta}_1,\,\boldsymbol{\beta}_2)$, the vector of causal coefficients for encoding linear effects of $ {X_{-k}}$ on outcome $Y$. 
Assume the unconfounded linear structural assignment $Y\coloneqq X_k \theta+X_{-k}^\top\boldsymbol{\beta}+U$, with $U$ zero mean random variable with finite variance $\sigma_U^2>0$, independent of $X$.} Then, 
%, independently of the $\boldsymbol{\gamma}$ parameters and of the functional form of the associated assignments between parents of $Y$
the score
\begin{equation}
   \psi( {W};\theta,\boldsymbol{\beta})=(Y-X_k\theta-X_{-k}^\top\boldsymbol{\beta})(X_k- {r}_{XX_{-k}} {X_{-k}})\,, \label{eq:score_without_expect}
\end{equation}
with $ {r}_{XX_{-k}}=\mathbb{E}[X_k  {X_{-k}}^\top]\mathbb{E}[ {X_{-k}}  {X_{-k}}^\top]^{-1}$,
follows the Neyman orthogonality condition for the estimation of $\theta$ with nuisance parameters $\boldsymbol{\eta}=(\beta,\boldsymbol{\gamma})$ which reads
\[
\mathbb{E}\left[(Y-X_k\theta- {X_{-k}}^\top\boldsymbol{\beta}) 
 (X_k-{r}_{XX_{-k}} {X_{-k}})\right]=0\,. \label{eq:lemma_3}
\]
\end{proposition}

  \begin{wrapfigure}{h}{0.45\textwidth}
            \centering
    \begin{tikzpicture}[
            > = stealth, % arrow head style
            shorten > = 1pt, % don't touch arrow head to node
            auto,
            node distance = 2.1cm, % distance between nodes
            semithick % line style
        ]

        \tikzstyle{every state}=[
            draw = black,
            thick,
            fill = white,
            minimum size = 7mm
        ]

        \node[state] (Y) {$Y$};
        \node[state] (Z1) [above right of=Y] {$ {Z}_1$};
        \node[state] (Z2) [right of=Z1] {$ {Z}_2$};
        \node[state] (Xk) [above of=Y,yshift=1cm] {$X_k$};
        %\node[state] (Y) [below right of=H] {$Y$};

        \path[->] (Xk) edge node {$\theta$} (Y);
       % \path[->] (s) edge node {1} (v);
        \path[->] (Z1) edge node [above] {$\beta_1$} (Y);
        \path[->] (Z2) edge node {$\beta_2$} (Y);
        \path[<->] (Xk) edge node [below] {$\boldsymbol{\gamma_1}$} (Z1);
        \path[<->] (Z2) edge node [above] {$\boldsymbol{\gamma}_2$} (Xk);
        \path[<->] (Z2) edge node [above] {$\boldsymbol{\gamma}_{12}$} (Z1);
        

       % \draw[red, dashed] (1, 2) -- (1, -2);
    \end{tikzpicture}
        \caption{A generic example of identification of a causal effect $\theta$ in the presence of causal and anti-causal interactions between the causal predictor and other putative parents, and possibly arbitrary cyclic and nonlinear assignments for all nodes except $Y$ (see Proposition~\ref{prp:general2var}). We have $X_{-k} = Z_1 \cup Z_2$.}
            \label{fig:general2var}
            %\vspace{-17mm}
\end{wrapfigure} 

Please refer to~\Cref{sec:infl_inter} for the proof.
\corrected{Applying \Cref{eq:debiasestim}, this leads to the debiased estimator
\[
\check \theta = \frac{\sum_i (Y_i- {X_{-k i}}^\top\boldsymbol{\check \beta}) 
 (X_{k i}-\check r_{XX_{-k}} {X_{-k}})}
 {\sum_{i} {X_{k i}}  
 (X_{k i}-\check r_{XX_{-k}} {X_{-k i}})}\,. \label{eq:lemma_3}
\]
which relies on ML estimates $\check{ \boldsymbol{\beta}}$ and $\check r_{XX_{-k}}$ .} 
Comparing the score in ~\Cref{eq:score_without_expect} with the score in~\Cref{eq:orthogonal_score}, there are two takeaways from Proposition~\ref{prp:general2var}: (i) the orthogonality condition remains invariant irrespective of the causal direction between $X_k$ and $Z$, and (ii) the second term in~\Cref{eq:lemma_3} replaces function $m$ by the (unbiased) linear regression estimator for modelling all the relations; given that the relation between $Z$ and $Y$ is linear, even if relationships between $Z$ and $X_k$ are non-linear (See~\Cref{app:example} for concrete examples). Combining with the Double ML theoretical results \citep{doubleml2016}, this suggests that regularized predictors based on Lasso or ridge regression are tools of choice for fitting functions $(m,g)$.
%\Cref{prp:general2var}  makes the simplifying assumption of Gaussianity to derive an explicit formula for the estimate of parameter theta using an orthogonalization approach based on the log-likelihood, as explained in section 2.2. However, the inference of causal parents relying on the following Prop. 3 does not rely on a Gaussianity assumption.

\subsection{Statistical Test} \label{subsec:test_stat}
%Now that we have illustrated and justified the fitting procedure of our algorithm, 
We now provide a theoretically grounded statistical decision criterion for the direct causes after the model has been fitted.
Consider $(Y,X)$, $Y\in\mathbb{R}$, $X\in\mathbb{R}^{d}$, satisfying
\begin{align}
    &Y=\langle \theta, X\rangle + U,
    \label{eq:model1}
    \\
    &\E(Y^{2})<\infty, ~ \E(U^{2})<\infty,  ~\E(U)=0,  \corrected{\E(U \mid X)=0,}  \text{~and } \E(\Vert X\Vert_{2}^{2})< \infty,
    \label{eq:model2}
    \\
    & \E\left[\left(X_{j} - \E(X_{j}\mid X_{-j}) \right)^{2}\right]\neq 0, \quad \text{for all }  j \in \lbrace 1,\dots,d\rbrace\,,
    \label{eq:model3}
\end{align}
where $U$ is an exogenous variable and $X_{-j}$ represents all the variables except ${X_j}$. The assumptions made with the above formulation are standard in the orthogonal machine learning literature \citep{rotnitzky2019characterization,smucler2019unifyin,NeweyCherno19}. They allow identifying causal parents based on estimates of conditional covariances $\chi_j$ defined in \Cref{eq:chi} %Let us define the quantity $\chi_{j}=\E\left[ \left(Y - \E(Y\mid X_{-j}) \right) \left(X_{j} - \E(X_{j}\mid X_{-j}) \right)\right]$ for $j \in \{1,\cdots, d \}$, which is the expected conditional covariance of $X_{j}$ given $X_{-j}$. 

\begin{proposition} \label{prp:main_exp}
Let $ PA_{Y} = \left\lbrace j\in \lbrace 1,\dots,d\rbrace : \theta_{j}\neq  0 \right\rbrace.$
%let $X_{-j}$ be the vector equals to $X$ but excluding coordinate $j$. 
%For  $j \in \lbrace 1,\dots,p\rbrace$
%$$
%\chi_{j}=\E\left[ \left(Y - \E(Y\mid X_{-j}) \right) \left(X_{j} - \E(X_{j}\mid %X_{-j}) \right)\right],
%$$
%which also 
%has the double robustness property \citep{NeweyCherno19,rotnitzky2019characterization} 
Then under the conditions given in~\Cref{eq:model1,eq:model2,eq:model3}, for each $j \in \lbrace 1,\dots,p\rbrace$ 
\begin{itemize}
    \item[a)] $\chi_{j}= \theta_{j} \E\left[\left(X_{j} - \E(X_{j}\mid X_{-j}) \right)^{2} \right]$ and $j\in PA_{Y}$ if and only if $\chi_{j}\neq 0$.
    \item[b)] We also have (with notations of Prop.~\ref{prp:general2var}) $
    \chi_{j}=\E\left[ \left(Y - \E(Y\mid X_{-j}) \right) \left(X_{j} -  {r}_{XX_{-j}} X_{-j}) \right)\right].
    $
\end{itemize}
\end{proposition}
The proof is given in \cref{appendix:prop3}.
There are two main implications of the results provided in Proposition~\ref{prp:main_exp}. (i) $\chi_j$ is non-zero only for direct causal parents of the outcome variable, and  $\chi_j$ has double robustness property as shown in \citep{rotnitzky2019characterization,smucler2019unifyin,NeweyCherno19}. Having double robustness property means that while computing the empirical version of the $\chi_j$ which we denote as $\hat{\chi}_j$, one can use regularized methods like ridge regression or Lasso to estimate the conditional expectation (function $m$). Afterward, one can perform statistical tests on top of it to decide between zero or non-zero tests. (ii) In line with the above orthogonal score results, we see that this quantity can be estimated using linear (unbiased) regression to fit the function $m$, although interactions between features may be non-linear.
Next, we discuss the variance of our estimator so that a statistical test can be used to identify causal parents. For the sake of convenience, the case of 2 partitions ($K=2$)\footnote{Extension to arbitrary number of data partitions ($K\geq2$) is straightforward. Check~\Cref{alg:double_ml_causal}.} is explained here.

\paragraph{Variance of Empirical Estimates of $\chi_j$:} Suppose we have $n$ i.i.d.\ observations indicated by $\mathcal{D}_{n}=\left\lbrace (X_{i},Y_{i}), i=1\dots,n \right\rbrace$. Randomly split the data in two halves, say $\mathcal{D}_{n1}$ and $\mathcal{D}_{n2}$.
Take $j\in \left\lbrace 1,\dots,d\right\rbrace$.
For $k=1$ let $\overline{k}=2$, for $k=2$ let $\overline{k}=1$. For $k=1,2$, compute estimates of
$
\widehat{\E}^{\overline{k}}\left( Y \mid X_{-j} \right) \quad \text{and} \quad \widehat{\E}^{\overline{k}}\left( X_{j} \mid X_{-j} \right)
$
using the data in sample $\overline{k}$. Following \cite{smucler2019unifyin}, we can use estimates of $\widehat{\E}^{\overline{k}}\left( Y \mid X_{-j} \right)$  and $\widehat{\E}^{\overline{k}}\left( X_{j} \mid X_{-j} \right)$ that are solutions of $\ell_1$-regularized regression problems to obtain square root N convergence guaranties. We  use Lasso as the estimator for conditional expectation in the experiments. Now, we compute the cross-fitted empirical estimates of $\chi_j$ and associated empirical variances
\begin{align}
\widehat{\chi}_{j}^{k}&=\mathbb{P}_{nk} \left[ -Y\widehat{\E}^{\overline{k}}\left( X_{j} \mid X_{-j} \right) - X_{j}\widehat{\E}^{\overline{k}}\left( Y \mid X_{-j} \right) + \widehat{\E}^{\overline{k}}\left( Y \mid X_{-j} \right)\widehat{\E}^{\overline{k}}\left( X_{j} \mid X_{-j} \right) + Y X_{j}\right]\label{eq:chi_bound}\\
\left(\widehat{\sigma}_{j}^{k}\right)^{2} &= \mathbb{P}_{nk} \left[ \left(-Y\widehat{\E}^{\overline{k}}\left( X_{j} \mid X_{-j} \right) - X_{j}\widehat{\E}^{\overline{k}}\left( Y \mid X_{-j} \right)  + \widehat{\E}^{\overline{k}}\left( Y \mid X_{-j} \right)\widehat{\E}^{\overline{k}}\left( X_{j} \mid X_{-j} \right) + Y X_{j}- \widehat{\chi}_{j}^{k} \right)^{2}\right]\,, \label{eq:var_bound}
\end{align}
where $\mathbb{P}_{nk}$ denotes the empirical average over the $k$ half.  Finally, let
\begin{equation}\label{eq:estimates}
\widehat{\chi}_{j} = \frac{1}{2}\left({\widehat{\chi}_{j}^{1} + \widehat{\chi}_{j}^{2}}\right), \quad \widehat{\sigma}_{j}^{2} = \frac{1}{2}\left( {\left(\widehat{\sigma}_{j}^{1}\right)^{2}  + \left(\widehat{\sigma}_{j}^{2}\right)^{2} }\right).
\end{equation}
 
 %\corrected{\citet{smucler2019unifyin} investigate the properties of $\ell_1$-regularised machine learning estimators for a particular family of non-parametric estimands, called Bilinear Influence Functionals (BIF). Our estimand of \Cref{eq:chi} belongs to this class as an expected conditional covariance \citep{smucler2019unifyin}[example 5] (see \Cref{app:doublerob} for more details).} 
 \correctedbis{Consistency of such estimators notably relies on sparsity assumptions for ground truth models in the asymptotic  high-dimensional setting where covariate dimension $p(=d-1)$ and sparsity is allowed to vary with number of samples $n$. In the notations below, we drop this dependency  and specialize to our case. 
%\begin{definition}[Approximate/Exact Linear-Sparse class (ALS/ELS)]
%Ground truth predictor $c(Z)$ belongs to the approximately sparse class whenever There exists $\theta^*\in \mathbb{R}^p$ and a function $r(Z)$ satisfying 
%$$
%c(Z) = \langle \theta^*,\phi(Z)\rangle +r(Z)
%$$
%where $\|\theta^*\|_0\leq s$ and $\E[r(Z)^2]\leq K(s\log(p)/n)$. When $r=0$, we talk about Exact Linear Sparse class (ELS).
%\end{definition}
\begin{definition}[Approximate Linear-Sparse class (ALS)]\label{def:als}
Ground truth predictor $c(X_{-j})$ belongs to the approximately sparse class whenever there exists $\theta^*\in \mathbb{R}^p$ and a function $r(X_{-j})$ satisfying 
$$
c(Z) = \langle \theta^*,\phi(Z)\rangle +r(Z)\,,\mbox{ where } \|\theta^*\|_0\leq s \mbox{ and } \E[r(Z)^2]\leq K(s\log(p)/n)\,. 
$$
\end{definition}
Theorem 1 of~\citep{smucler2019unifyin} provides general conditions under which (see also \citep{NeweyCherno19}), when the estimators
%\begin{align}
$\widehat{\E}^{\overline{k}}\left( Y \mid X_{-j} \right) \quad$ and  $\widehat{\E}^{\overline{k}}\left( X_{j} \mid X_{-j} \right)$ are Lasso-type regularized linear regressions. 
%In particular, the following conditions are sufficient for 
%$\widehat{\chi}_{j} \approx \mathcal{N}\left(\chi_{j}, \frac{\widehat{\sigma}_{j}^{2} }{n}\right)$ to hold asymptotically.
}  
\begin{proposition}\label{prop:doublerob}
\correctedbis{Given eqs. (\ref{eq:model1}-\ref{eq:model3}) and $j\in \{1,...,d\}$. Assume: (i) For true parameter in~(\ref{eq:model1}), $\|\theta\|_0\leq s$ with $s\log(p)/n\to 0$; (ii) ${r}_{XX_{-j}} X_{-j}$ is in the ALS class with $s\log(p)/n\to 0$; (iii) All $X_k$ have support bounded by the same constant; (iv) $U$ is independent of $X$ and has tail decaying at least as fast as an exponential random variable; (v) $\E[X_{-j}X_{-j}^\top]$ has eigenvalues lower and upper bounded; (vi) $\E[Y-\E[Y|X_{-j}]|X_{-j}]$ and $\E[X_j-\E[X_j|X_{-j}]|X_{-j}]$ are bounded with variance lower bounded.\newline
Then the pair of estimators $(\widehat{\chi}_j,\,\widehat{\sigma}^2_j)$ of eq.~(\ref{eq:estimates}), using $l_1$ regularization coefficient $\lambda \approx \sqrt{\log(p)/n}$ for both Lasso estimates, satisfies   
$
\widehat{\chi}_j \overset{D}{\to}  \mathcal{N}\left(\chi_{j}, \frac{\widehat{\sigma}_{j}^{2} }{n}\right)\,.
$, as $n\to +\infty$.}
\end{proposition}
\correctedbis{All stated bounds are uniform across $n$ and strictly positive. Proof is provided in Appendix~\ref{app:doublerob} with the broader context on the doubly robust estimation framework. The provided conditions correspond to a concise special case of the general statements provided in \cite{smucler2019unifyin}. It is possible to relax some of these assumptions, notably to allow some misspecifications of the sparsity assumptions for the Lasso estimates. Overall, the mildness of these assumptions may explain the empirical success of this approach in the following section.} 

Under conditions of \cref{prop:doublerob}, the test that rejects $\chi_{j}=0$ when 
$ \vert \widehat{\chi}_{j} \vert \geq 1.96 \frac{\widehat{\sigma}_{j}}{\sqrt{n}} $
will have approximately $95\%$ confidence level. The probability of rejecting the null when it is false is 
\begin{align*}
P\left( \vert \widehat{\chi}_{j} \vert \geq 1.96 \frac{\widehat{\sigma}_{j}}{\sqrt{n}} \right) \geq P\left( \vert \widehat{\chi}_{j} - \chi_{j}\vert \leq \vert \chi_{j}\vert - 1.96 \frac{\widehat{\sigma}_{j}}{\sqrt{n}} \right)  \to 1.
\end{align*}
In order to account for multiple testing, we use Bonferroni correction.

%\paragraph{Comments about Estimator:}
 % In this paper, we use Lasso for the nuisance parameter estimation as the variance of the conditional covariance is known~\citep{smucler2019unifyin}. One can also use other estimators instead, assuming one obtains a reasonable enough estimate of the nuisance parameter (up to $N^{-1/4}$-neighbourhood~\citep{doubleml2016}) with the correct variance term, which is beyond the scope of this paper.
  
 \paragraph{Conditional Independence Tests:} Asymptotically, the conditional independence testing between $Y$ and $X_j$ given $X_{-j}$ is also a possible solution for our proposed approach. Indeed, d-separation rules imply that true causes are conditionally dependent according to this test, while non-causes are conditionally independent (because $X_{-j}$ is not a collider under our NFD assumption). However, conditional independence testing is challenging in high-dimensional/non-linear settings. Kernel-based conditional independence testing is computationally expensive~\citep{zhang2012kernel}. We used $\chi_j$ in the paper because it was already known from previous works ~\citep{smucler2019unifyin,doubleriesz2018} that it has double robustness property, which means one can use regularized methods like Lasso to estimate empirical conditional expectation from a finite number of samples and the empirical estimator is still unbiased with controlled variance. Our work is related to the recent work of~\citep{shah2020hardness}, which proposes a conditional independence test whose proofs rely heavily on \citep{doubleml2016}. In this paper, we use for the first time such double ML-based tests for the search problem.




==> TMLR 2022_ Causal Feature Selection via Orthogonal Search 2/notation.tex <==
% \DeclareMathOperator*{\argmin}{arg\,min}
% \DeclareMathOperator*{\argmax}{arg\,max}

\def\R{{\mathbb{R}}}

\newcommand{\abs}[1]{{\left\lvert#1\right\rvert}}
\newcommand{\norm}[1]{{ \left\lVert#1\right\rVert }}
\newcommand{\EE}[1]{ \mathbb{E}\left[#1\right] }

\def\bbE{{\mathbb{E}}}
\def\E{{\mathbb{E}}}
\def\cO{{\mathcal{O}}}

\makeatletter
\def\blfootnote{\gdef\@thefnmark{}\@footnotetext}
\makeatother

%for comments
\newcommand{\stefan}[1]{{{\color{red} Stefan: #1}}}
\newcommand{\anant}[1]{{{\color{blue} Anant: #1}}}
\newcommand{\bernhard}[1]{{{\color{green} Bernhard: #1}}}
\newcommand{\ashkan}[1]{{{\color{cyan} Ashkan: #1}}}
\newcommand{\michel}[1]{{{\color{orange} Michel: #1}}}

% \newcommand{\corrected}[1]{\textcolor{red}{#1}}
% \newcommand{\correctedbis}[1]{\textcolor{teal}{#1}}

\newcommand{\corrected}[1]{#1}
\newcommand{\correctedbis}[1]{#1}



==> TMLR 2022_ Causal Feature Selection via Orthogonal Search 2/requirements.tex <==
\usepackage{wrapfig}
\usepackage{lipsum}
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{soul,xcolor}
\usepackage{algorithm}

\usepackage{chngcntr}
\usepackage{etoolbox}

% save the meaning of \AND and undefine it to keep algorithmic happy
\let\classAND\AND
\let\AND\relax
% load algorithmic
\usepackage{algorithmic}

% save the new meaning of \AND and restore the one of the class
\let\algoAND\AND
\let\AND\classAND
%% but when we start \begin{algorithmic} we want its own \AND
\AtBeginEnvironment{algorithmic}{\let\AND\algoAND}


\usepackage{enumitem}

\usepackage{pgf,tikz} % graphical models
\usetikzlibrary{bayesnet}
\usetikzlibrary{positioning}
\usepackage{tikz-dependency}
\usetikzlibrary{arrows, automata}

\usepackage{caption}
\usepackage{subcaption}

\usepackage{multirow}
\usepackage{cleveref}

\usepackage{booktabs}
\usepackage{float}
\usepackage{chngcntr}


\usepackage{longtable}

\usepackage{lipsum}



==> TMLR 2022_ Causal Feature Selection via Orthogonal Search 2/tables.tex <==
\begin{table*}[!ht]
    \footnotesize
	\caption[Caption for LOF]{Performance across all the settings for different number of nodes. Each single entry in the table is averaged over 18000 simulations. Our method is almost state of the art in every case.}
	\label{Table_Number_of_Nodes}
	\centering
	\setlength{\tabcolsep}{4pt}
	\begin{tabular}{ l c c c|c c c|c c c|c c c} %@{\extracolsep{\fill}}
		\toprule
		& \multicolumn{12}{c}{Number of Nodes} \\
		\hline
		\multirow{2}{*}{Method} & \multicolumn{3}{c}{5} & \multicolumn{3}{c}{10} & \multicolumn{3}{c}{20} & \multicolumn{3}{c}{50} \\
		\multicolumn{1}{c}{} & ACC & CSI & F1 & ACC & CSI & F1 & ACC & CSI & F1 & ACC & CSI & F1 \\
		\midrule
		%\hline
		%\hline
		GES & 0.935 & 0.890 & 0.911 & 0.854 & 0.730 & 0.779 & 0.743 & 0.442 & 0.526 & 0.698 & 0.245 & 0.323 \\
		rankGES & 0.923 & 0.857 & 0.883 & 0.846 & 0.700 & 0.753 & 0.740 & 0.428 & 0.514 & 0.697 & 0.237 & 0.316 \\
	%	\hline
	%	\hline
		ARGES & 0.922 & 0.864 & 0.885 & 0.797 & 0.551 & 0.584 & 0.752 & 0.447 & 0.524 & 0.705 & 0.186 & 0.221 \\
		rankARGES & 0.914 & 0.838 & 0.861 & 0.793 & 0.537 & 0.572 & 0.750 & 0.435 & 0.514 & 0.705 & 0.181 & 0.216 \\
	%	\hline
	%	\hline
		FCI+ & 0.963 & 0.918 & 0.932 & 0.873 & 0.744 & 0.808 & 0.830 & 0.602 & 0.703 & 0.766 & 0.368 & 0.486 \\
	%	\hline
	%	\hline
		LINGAM & \textbf{0.991} & \textbf{0.978} & \textbf{0.982} & \textbf{0.953} & 0.865 & 0.889 & 0.891 & 0.712 & 0.778 & 0.750 & 0.318 & 0.385 \\
	%	\hline
	%	\hline
		PC & 0.957 & 0.913 & 0.929 & 0.864 & 0.723 & 0.786 & 0.823 & 0.569 & 0.664 & 0.763 & 0.348 & 0.457 \\
		rankPC & 0.946 & 0.891 & 0.912 & 0.854 & 0.701 & 0.768 & 0.813 & 0.541 & 0.638 & 0.754 & 0.324 & 0.431 \\
	%	\hline 
	%	\hline 
    	MMPC & 0.868 & 0.586 & 0.597 & 0.823 & 0.494 & 0.535 & 0.790 & 0.412 & 0.489 & 0.749 & 0.260 & 0.350 \\
    	%	\hline 
    	%	\hline
		MMHC & 0.929 & 0.878 & 0.905 & 0.841 & 0.675 & 0.739 & 0.767 & 0.432 & 0.507 & 0.725 & 0.218 & 0.281 \\
	%	\hline 
	%	\hline
	    GS & 0.883 & 0.613 & 0.623 & 0.855 & 0.563 & 0.601 & 0.824 & 0.501 & 0.580 & 0.759 & 0.310 & 0.388 \\
		%\hline 
		%\hline
		IAMB & 0.850 & 0.571 & 0.585 & 0.791 & 0.508 & 0.561 & 0.806 & 0.500 & 0.587 & 0.768 & 0.337 & 0.424 \\
		%\hline 
		%\hline
		FastIAMB & 0.883 & 0.614 & 0.624 & 0.858 & 0.571 & 0.611 & 0.828 & 0.511 & 0.593 & 0.770  & 0.326 & 0.409 \\
		%\hline 
		%\hline
		IAMB-FDR & 0.869 & 0.584 & 0.593 & 0.831 & 0.494 & 0.526 & 0.825 & 0.484 & 0.558 & 0.770 & 0.322 & 0.406 \\
		%\hline 
		%\hline
		PCI & 0.984 & 0.965 & 0.972 & 0.922 & 0.844 & 0.875 & 0.888 & 0.734 & 0.782 & 0.773 & 0.414 & 0.491 \\
		%\hline 
	    %\hline
		Lasso & 0.965 & 0.948 & 0.968 & 0.905 & 0.834 & 0.892 & 0.894 & 0.786 & 0.866 & 0.773 & 0.489 & 0.627 \\
		\texttt{CORTH Features (Ours)} & 0.988 & 0.968 & 0.973 & 0.949 & \textbf{0.908} & \textbf{0.934} & \textbf{0.949} & \textbf{0.865} & \textbf{0.905} & \textbf{0.795} & \textbf{0.559} & \textbf{0.663} \\
		\midrule
	%	\hline
	%	\hline
		& \multicolumn{12}{c}{Number of Nodes} \\
		\midrule
		\multirow{2}{*}{Method} & \multicolumn{3}{c}{5} & \multicolumn{3}{c}{10} & \multicolumn{3}{c}{20} & \multicolumn{3}{c}{50} \\
		\multicolumn{1}{c}{} & TPR & FPR & MCC & TPR & FPR & MCC & TPR & FPR & MCC & TPR & FPR & MCC \\
		\midrule
	%	\hline
	%	\hline
		GES & 0.934 & 0.056 & 0.891 & 0.790 & 0.090 & 0.711 & 0.502 & 0.088 & 0.436 & 0.304 & 0.083 & 0.221 \\
		rankGES & 0.924 & 0.068 & 0.877 & 0.780 & 0.098 & 0.695 & 0.493 & 0.089 & 0.425 & 0.297 & 0.083 & 0.215 \\
		%\hline
		%\hline
		ARGES & 0.903 & 0.046 & 0.906 & 0.590 & 0.041 & 0.841 & 0.500 & 0.073 & 0.557 & 0.220 & 0.020 & 0.794 \\
		rankARGES & 0.897 & 0.054 & 0.896 & 0.584 & 0.044 & 0.832 & 0.495 & 0.075 & 0.549 & 0.216 & 0.020 & 0.789 \\
		%\hline
		%\hline
		FCI+ & 0.969 & 0.029 & 0.948 & 0.797 & 0.054 & 0.759 & 0.642 & 0.042 & 0.645 & 0.389 & 0.030 & 0.454 \\
		%\hline
		%\hline
		LINGAM & 0.991 & 0.007 & 0.988 & 0.886 & 0.008 & 0.934 & 0.770 & 0.055 & 0.759 & 0.391 & 0.072 & 0.471 \\
		%\hline
		%\hline
		PC & 0.950 & 0.024 & 0.941 & 0.759 & 0.041 & 0.759 & 0.600 & 0.032 & 0.650 & 0.363 & 0.021 & 0.468 \\
		rankPC & 0.944 & 0.039 & 0.925 & 0.750 & 0.053 & 0.734 & 0.580 & 0.034 & 0.629 & 0.341 & 0.024 & 0.427 \\
		%\hline 
		%\hline 
		MMPC & 0.588 & 0.006 & 0.965 & 0.498 & 0.011 & 0.852 & 0.417 & 0.006 & 0.684 & 0.261 & 0.003 & 0.528 \\
    	%	\hline 
    	%	\hline
		MMHC & 0.895 & 0.011 & 0.903 & 0.691 & 0.015 & 0.724 & 0.444 & 0.009 & 0.523 & 0.219 & 0.005 & 0.330 \\
		%\hline 
		%\hline
		GS & 0.615 & 0.002 & 0.973 & 0.566 & 0.001 & 0.895 & 0.506 & 0.001 & 0.739 & 0.311 & 0.000 & 0.688 \\
		%\hline 
		%\hline
		IAMB & 0.573 & 0.003 & 0.960 & 0.511 & 0.002 & 0.848 & 0.505 & 0.001 & 0.711 & 0.338 & 0.001 & 0.660 \\
		%\hline 
		%\hline
		FastIAMB & 0.616 & 0.003 & 0.972 & 0.575 & 0.002 & 0.888 & 0.518 & 0.002 & 0.734 & 0.327  & 0.001 & 0.677 \\
		%\hline 
		%\hline
		IAMB-FDR & 0.585 & 0.001 & 0.975 & 0.494 & 0.001 & 0.909 & 0.485 & 0.001 & 0.766 & 0.322 & 0.001 & 0.661 \\
		%\hline 
		%\hline
		PCI & 0.992 & 0.017 & 0.981 & 0.875 & 0.028 & 0.890 & 0.754 & 0.016 & 0.839 & 0.430 & 0.030 & 0.638 \\
		%\hline 
		%\hline
		Lasso & 0.999 & 0.074 & 0.949 & 0.944 & 0.119 & 0.817 & 0.954 & 0.147 & 0.794 & 0.681 & 0.148 & 0.488 \\
		\texttt{CORTH Features (Ours)} & 0.999 & 0.016 & 0.986 & 0.952 & 0.044 & 0.906 & 0.884 & 0.011 & 0.894 & 0.609 & 0.101 & 0.567 \\
		\bottomrule
		\end{tabular}
\end{table*}


\begin{table*}[!ht]
    \footnotesize
	%increase table row spacing, adjust to taste
% 	\renewcommand{\arraystretch}{1.3}
	%if using array.sty, it might be a good idea to tweak the value of
	% \extrarowheight as needed to properly center the text within the cells
	%\captionsetup{font=small}
	\caption[Caption for LOF]{Performance across all the settings for different number of nonlinear probabilities. Each single entry in the table is averaged over 18000 simulations. Our method is almost state of the art in every case.}
	\label{Table_Nonlinearity}
	\centering
	\setlength{\tabcolsep}{4pt}
	% Some packages, such as MDW tools, offer better commands for making tables
	% than the plain LaTeX2e tabular which is used here.
	\begin{tabular}{ l c c c|c c c|c c c|c c c} %@{\extracolsep{\fill}}
		\toprule
		& \multicolumn{12}{c}{Nonlinear Probability} \\
		\hline
		\multirow{2}{*}{Method} & \multicolumn{3}{c}{0} & \multicolumn{3}{c}{0.3} & \multicolumn{3}{c}{0.5} & \multicolumn{3}{c}{1} \\
		\multicolumn{1}{c}{} & ACC & CSI & F1 & ACC & CSI & F1 & ACC & CSI & F1 & ACC & CSI & F1 \\
		\midrule
	%	\hline
	%	\hline
		GES & 0.803 & 0.583 & 0.646 & 0.806 & 0.566 & 0.622 & 0.811 & 0.577 & 0.632 & 0.810 & 0.581 & 0.641 \\
		rankGES & 0.796 & 0.559 & 0.625 & 0.801 & 0.546 & 0.605 & 0.805 & 0.556 & 0.613 & 0.805 & 0.561 & 0.623 \\
	%	\hline
	%	\hline
		ARGES & 0.781 & 0.476 & 0.515 & 0.786 & 0.486 & 0.525 & 0.792 & 0.506 & 0.546 & 0.818 & 0.581 & 0.628 \\
		rankARGES & 0.778 & 0.461 & 0.503 & 0.782 & 0.474 & 0.515 & 0.788 & 0.490 & 0.531 & 0.814 & 0.564 & 0.615 \\
		%\hline
		%\hline
		FCI+ & 0.827 & 0.599 & 0.674 & 0.860 & 0.663 & 0.745 & 0.872 & 0.685 & 0.764 & 0.873 & 0.685 & 0.746 \\
		%\hline
		%\hline
		LINGAM & \textbf{0.907} & 0.738 & 0.778 & 0.886 & 0.689 & 0.725 & 0.880 & 0.684 & 0.724 & 0.911 & 0.762 & 0.808 \\
	%	\hline
	%	\hline
		PC & 0.818 & 0.574 & 0.641 & 0.854 & 0.641 & 0.720 & 0.864 & 0.665 & 0.7430 & 0.869 & 0.672 & 0.731 \\
		rankPC & 0.813 & 0.560 & 0.630 & 0.841 & 0.614 & 0.694 & 0.848 & 0.627 & 0.704 & 0.864 & 0.656 & 0.720 \\
	%	\hline 
	%	\hline
        MMPC & 0.775 & 0.372 & 0.416 & 0.809 & 0.439 & 0.503 & 0.818 & 0.462 & 0.528 & 0.828 & 0.479 & 0.523 \\
    	%	\hline 
    	%	\hline
		MMHC & 0.797 & 0.516 & 0.578 & 0.815 & 0.549 & 0.610 & 0.823 & 0.566 & 0.625 & 0.826 & 0.571 & 0.620 \\
	%	\hline 
	%	\hline
    	GS & 0.806 & 0.450 & 0.491 & 0.828 & 0.494 & 0.554 & 0.835 & 0.510 & 0.571 & 0.851 & 0.534 & 0.576 \\
    	%	\hline 
    	%	\hline
    	IAMB & 0.762 & 0.389 & 0.440 & 0.799 & 0.463 & 0.538 & 0.809 & 0.488 & 0.565 & 0.830 & 0.520 & 0.576 \\
		%\hline 
		%\hline
		FastIAMB & 0.807 & 0.454 & 0.497 & 0.835 & 0.503 & 0.566 & 0.842 & 0.522 & 0.587 & 0.855  & 0.543 & 0.587 \\
		%\hline 
		%\hline
		IAMB-FDR & 0.796 & 0.418 & 0.457 & 0.818 & 0.456 & 0.511 & 0.827 & 0.481 & 0.538 & 0.853 & 0.529 &  0.578 \\
		%\hline 
		%\hline
		PCI & 0.853 & 0.674 & 0.720 & 0.897 & 0.746 & 0.789 & 0.905 & 0.763 & 0.806 & 0.911 & 0.774 & 0.805 \\
	    %\hline 
	    %\hline
		Lasso & 0.847 & 0.694 & 0.773 & 0.891 & 0.776 & 0.853 & 0.902 & 0.797 & 0.869 & 0.896 & 0.790 & 0.857 \\
		\texttt{CORTH Features (Ours)} & 0.871 & \textbf{0.768} & \textbf{0.824} & \textbf{0.934} & \textbf{0.830} & \textbf{0.873} & \textbf{0.943} & \textbf{0.851} & \textbf{0.891} & \textbf{0.933} & \textbf{0.852} & \textbf{0.887} \\
		%\hline
		%\hline
		& \multicolumn{12}{c}{Nonlinear Probability} \\
		\hline
		\multirow{2}{*}{Method} & \multicolumn{3}{c}{0} & \multicolumn{3}{c}{0.3} & \multicolumn{3}{c}{0.5} & \multicolumn{3}{c}{1} \\
		\multicolumn{1}{c}{} & TPR & FPR & MCC & TPR & FPR & MCC & TPR & FPR & MCC & TPR & FPR & MCC \\
		%\hline
	%	\hline
		GES & 0.643 & 0.093 & 0.564 & 0.620 & 0.074 & 0.557 & 0.629 & 0.071 & 0.568 & 0.637 & 0.079 & 0.570 \\
		rankGES & 0.633 & 0.100 & 0.550 & 0.612 & 0.080 & 0.546 & 0.620 & 0.076 & 0.557 & 0.628 & 0.083 & 0.559 \\
		%\hline
	%	\hline
		ARGES & 0.514 & 0.041 & 0.789 & 0.526 & 0.041 & 0.793 & 0.547 & 0.043 & 0.791 & 0.626 & 0.055 & 0.725 \\
		rankARGES & 0.509 & 0.044 & 0.780 & 0.522 & 0.044 & 0.788 & 0.540 & 0.046 & 0.783 & 0.620 & 0.059 & 0.715 \\
	%	\hline
	%	\hline
		FCI+ & 0.638 & 0.045 & 0.637 & 0.704 & 0.037 & 0.708 & 0.728 & 0.035 & 0.731 & 0.728 & 0.037 & 0.730 \\
	%	\hline
	%	\hline
		LINGAM & 0.775 & 0.025 & 0.832 & 0.723 & 0.028 & 0.759 & 0.722 & 0.034 & 0.741 & 0.819 & 0.053 & 0.822 \\
	%	\hline
	%	\hline
		PC & 0.605 & 0.037 & 0.649 & 0.672 & 0.027 & 0.707 & 0.695 & 0.025 & 0.728 & 0.702 & 0.029 & 0.734 \\
		rankPC & 0.597 & 0.043 & 0.626 & 0.656 & 0.040 & 0.680 & 0.668 & 0.036 & 0.695 & 0.692 & 0.031 & 0.714 \\
	%	\hline 
	%	\hline 
	    MMPC & 0.376 & 0.009 & 0.754 & 0.442 & 0.006 & 0.738 & 0.465 & 0.005 & 0.749 & 0.482 & 0.005 & 0.787 \\
    	%	\hline 
    	%	\hline
		MMHC & 0.528 & 0.017 & 0.581 & 0.561 & 0.008 & 0.623 & 0.578 & 0.007 & 0.636 & 0.582 & 0.008 & 0.639 \\
		%\hline 
		%\hline
		GS & 0.452 & 0.001 & 0.850 & 0.496 & 0.001 & 0.797 & 0.513 & 0.001 & 0.799 & 0.538 & 0.001 & 0.849 \\
    	%	\hline 
    	%	\hline
    	IAMB & 0.847 & 0.003 & 0.773 & 0.891 & 0.002 & 0.853 & 0.902 & 0.001 & 0.869 & 0.896 & 0.001 & 0.857 \\
		%\hline 
		%\hline
		FastIAMB & 0.457 & 0.001 & 0.848 & 0.506 & 0.002 & 0.784 & 0.526 & 0.002 & 0.791 & 0.548 & 0.002 & 0.848 \\
		%\hline 
		%\hline
		IAMB-FDR & 0.418 & 0.001 & 0.837 & 0.457 & 0.001 & 0.819 & 0.481 & 0.001 & 0.822 & 0.530 & 0.001 & 0.833 \\
		%\hline 
		%\hline
		PCI & 0.712 & 0.057 & 0.792 & 0.765 & 0.011 & 0.848 & 0.781 & 0.010 & 0.845 & 0.794 & 0.013 & 0.864 \\
		%\hline 
		%\hline
		Lasso & 0.823 & 0.130 & 0.684 & 0.907 & 0.120 & 0.778 & 0.926 & 0.116 & 0.800 & 0.921 & 0.122 & 0.787 \\
		\texttt{CORTH Features (Ours)} & 0.840 & 0.119 & 0.730 & 0.849 & 0.007 & 0.872 & 0.870 & 0.008 & 0.888 & 0.885 & 0.038 & 0.863 \\
		\bottomrule
		\end{tabular}
\end{table*}



\begin{table*}[!ht]
    \footnotesize
	\caption[Caption for LOF]{Performance across all the settings for different connectivities. Each single entry in the table is averaged over 24000 simulations. Our method is almost state of the art in every case.}
	\label{Table_Sparsity}
	\centering
	\setlength{\tabcolsep}{4.03pt}
	\begin{tabular}{ l r r r  r | r r r r|  r r r r} %@{\extracolsep{\fill}}
		\toprule
		& \multicolumn{12}{c}{Connectivity} \\
		\hline
		\multirow{2}{*}{Method} & \multicolumn{4}{c}{0.1} & \multicolumn{4}{c}{0.3} & \multicolumn{4}{c}{0.5}\\
		\multicolumn{1}{c}{} & ACC & CSI & F1 & MCC & ACC & CSI & F1 & MCC & ACC & CSI & F1 & MCC \\
		\midrule
	%	\hline
	%	\hline
		GES & 0.961 & 0.786 & 0.825 & 0.857 & 0.815 & 0.539 & 0.598 & 0.522 & 0.646 & 0.405 & 0.482 & 0.315 \\
		rankGES & 0.954 & 0.746 & 0.790 & 0.840 & 0.809 & 0.522 & 0.584 & 0.511 & 0.642 & 0.398 & 0.475 & 0.308 \\
		%\hline
		%\hline
		ARGES & 0.965 & 0.794 & 0.828 & 0.876 & 0.805 & 0.456 & 0.501 & 0.726 & 0.612 & 0.286 & 0.330 & 0.720 \\
		rankARGES & 0.959 & 0.763 & 0.801 & 0.863 & 0.802 & 0.447 & 0.494 & 0.721 & 0.611 & 0.282 & 0.328 & 0.716 \\
		%\hline
		%\hline
		FCI+ & 0.974 & 0.819 & 0.853 & 0.910 & 0.866 & 0.631 & 0.714 & 0.674 & 0.734 & 0.524 & 0.629 & 0.521 \\
		%\hline
		%\hline
		LINGAM & 0.966 & 0.763 & 0.796 & 0.889 & 0.896 & 0.710 & 0.753 & 0.761 & 0.827 & 0.682 & 0.727 & 0.715 \\
		%\hline
		%\hline
		PC & 0.975 & 0.819 & 0.849 & 0.921 & 0.861 & 0.609 & 0.689 & 0.676 & 0.718 & 0.486 & 0.588 & 0.516 \\
		rankPC & 0.971 & 0.797 & 0.831 & 0.912 & 0.852 & 0.587 & 0.670 & 0.653 & 0.701 & 0.458 & 0.560 & 0.470 \\
		%\hline 
		%\hline 
		MMPC & 0.949 & 0.606 & 0.637 & 0.901 & 0.815 & 0.390 & 0.451 & 0.722 & 0.658 & 0.318 & 0.389 & 0.648 \\
		%\hline 
		%\hline
		MMHC & 0.978 & 0.834 & 0.867 & 0.901 & 0.830 & 0.497 & 0.561 & 0.574 & 0.639 & 0.321 & 0.397 & 0.385 \\
		%\hline 
		%\hline
		GS & 0.954 & 0.644 & 0.669 & 0.935 & 0.843 & 0.467 & 0.524 & 0.815 & 0.693 & 0.380 & 0.451 & 0.722 \\
		%\hline 
		%\hline
		IAMB & 0.969 & 0.692 & 0.745 & 0.864 & 0.841 & 0.463 & 0.522 & 0.807 & 0.692 & 0.377 & 0.452 & 0.709 \\
		%\hline 
		%\hline
		FastIAMB & 0.955 & 0.650 & 0.676 & 0.931 & 0.845 & 0.474 & 0.535 & 0.804 & 0.705 & 0.392 & 0.467 & 0.718 \\
		%\hline 
		%\hline
		IAMB-FDR & 0.950 & 0.608 & 0.626 & 0.961 & 0.832 & 0.436 & 0.492 & 0.816 & 0.689 & 0.369 & 0.446 & 0.707 \\
		%\hline 
		%\hline
		PCI & 0.986 & 0.902 & 0.920 & 0.954 & 0.906 & 0.716 & 0.759 & \textbf{0.838} & 0.783 & 0.600 & 0.661 & 0.720 \\
	    %\hline 
	    %\hline
		Lasso & 0.976 & 0.886 & 0.925 & 0.926 & 0.876 & 0.725 & 0.811 & 0.737 & 0.800 & 0.682 & 0.778 & 0.622 \\
		\texttt{CORTH Features (Ours)} & \textbf{0.988} & \textbf{0.915} & \textbf{0.934} & \textbf{0.959} & \textbf{0.926} & \textbf{0.813} & \textbf{0.858} & 0.833 & \textbf{0.847} & \textbf{0.747} & \textbf{0.814} & \textbf{0.724} \\
		\hline
		\end{tabular}
\end{table*}



\begin{table*}[!ht]
    \footnotesize
	\caption[Caption for LOF]{Performance across all the settings for different noise levels. Each single entry in the table is averaged over 14400 simulations. Our method is almost state of the art in every case.}
	\label{Table_Noise}
	\centering
	\setlength{\tabcolsep}{4.12pt}
	\begin{tabular}{ l c c c c | c c c c | c c c c} %@{\extracolsep{\fill}}
		\toprule
		& \multicolumn{12}{c}{Noise Level} \\
		\midrule
		\multirow{2}{*}{Method} & \multicolumn{4}{c}{0.01} & \multicolumn{4}{c}{0.5} & \multicolumn{4}{c}{1}\\
		\multicolumn{1}{c}{} & ACC & CSI & F1 & MCC & ACC & CSI & F1 & MCC & ACC & CSI & F1 & MCC \\
		\midrule
		%\hline
		%\hline
		GES & 0.804 & 0.579 & 0.639 & 0.559 & 0.808 & 0.571 & 0.629 & 0.562 & 0.818 & 0.586 & 0.644 & 0.589 \\
		rankGES & 0.797 & 0.557 & 0.619 & 0.548 & 0.802 & 0.552 & 0.613 & 0.551 & 0.812 & 0.565 & 0.625 & 0.577 \\
		%\hline
		%\hline
		ARGES & 0.810 & 0.572 & 0.625 & 0.653 & 0.789 & 0.496 & 0.534 & 0.814 & 0.774 & 0.434 & 0.460 & 0.897 \\
		rankARGES & 0.804 & 0.549 & 0.605 & 0.643 & 0.786 & 0.483 & 0.523 & 0.806 & 0.774 & 0.433 & 0.459 & 0.895 \\
		%\hline
		%\hline
		FCI+ & 0.843 & 0.617 & 0.691 & 0.674 & 0.865 & 0.678 & 0.753 & 0.717 & 0.874 & 0.697 & 0.766 & 0.740 \\
		%\hline
		%\hline
		LINGAM & 0.888 & 0.703 & 0.744 & 0.763 & 0.899 & 0.723 & 0.763 & 0.797 & 0.903 & 0.732 & 0.773 & 0.803 \\
		%\hline
		%\hline
		PC & 0.837 & 0.595 & 0.664 & 0.683 & 0.859 & 0.659 & 0.731 & 0.716 & 0.870 & 0.686 & 0.752 & 0.745 \\
		rankPC & 0.831 & 0.584 & 0.657 & 0.653 & 0.845 & 0.626 & 0.699 & 0.688 & 0.856 & 0.655 & 0.724 & 0.714 \\
		%\hline 
		%\hline
		MMPC & 0.796 & 0.405 & 0.456 & 0.762 & 0.812 & 0.453 & 0.510 & 0.756 & 0.825 & 0.480 & 0.533 & 0.780 \\
		%\hline 
		%\hline
		MMHC & 0.806 & 0.526 & 0.585 & 0.605 & 0.818 & 0.557 & 0.615 & 0.626 & 0.829 & 0.586 & 0.639 & 0.652 \\
		%\hline 
		%\hline
		GS & 0.820 & 0.468 & 0.518 & \textbf{0.824} & 0.836 & 0.513 & 0.566 & 0.819 & 0.846 & 0.538 & 0.586 & 0.833 \\
    	%\hline 
    %	\hline
        IAMB & 0.784 & 0.421 & 0.483 & 0.779 & 0.807 & 0.485 & 0.552 & 0.769 & 0.823 & 0.523 & 0.586 & 0.790 \\
		%\hline 
		%\hline
		FasIAMB & 0.821 & 0.469 & 0.520 & 0.819 & 0.842 & 0.526 & 0.582 & 0.814 & 0.852 & 0.548 & 0.600 & 0.828 \\
		%\hline 
		%\hline
		IAMB-FDR & 0.810 & 0.432 & 0.478 & 0.834 & 0.831 & 0.492 & 0.545 & 0.825 & 0.841 & 0.514 & 0.563 & 0.841 \\
		%\hline 
		%\hline
		PCI & 0.873 & 0.690 & 0.730 & 0.819 & 0.901 & 0.760 & 0.801 & 0.846 & 0.906 & 0.777 & 0.815 & 0.854 \\
		%\hline 
	    %\hline
		Lasso & 0.868 & 0.728 & 0.807 & 0.725 & 0.891 & 0.780 & 0.852 & 0.779 & 0.898 & 0.794 & 0.861 & 0.793 \\
		\texttt{CORTH Features (Ours)} & \textbf{0.899} & \textbf{0.789} & \textbf{0.839} & 0.795 & \textbf{0.929} & \textbf{0.842} & \textbf{0.883} & \textbf{0.858} & \textbf{0.934} & \textbf{0.854} & \textbf{0.891} & \textbf{0.866} \\
		\bottomrule
		\end{tabular}
\end{table*}


\begin{table*}[!ht]
    \footnotesize
	\caption[Caption for LOF]{Performance across all the settings for different number of observations. Each single entry in the table is averaged over 24000 simulations. Our method is almost state of the art in every case.}
	\label{Table_Observation}
	\centering
	\setlength{\tabcolsep}{4.12pt}
	\begin{tabular}{ l c c c c | c c c c | c c c c} %@{\extracolsep{\fill}}
		\toprule
		& \multicolumn{12}{c}{Number of Observations} \\
		\hline
		\multirow{2}{*}{Method} & \multicolumn{4}{c}{100} & \multicolumn{4}{c}{500} & \multicolumn{4}{c}{1000}\\
		\multicolumn{1}{c}{} & ACC & CSI & F1 & MCC & ACC & CSI & F1 & MCC & ACC & CSI & F1 & MCC \\
		\midrule
		%\hline
		%\hline
		GES & 0.797 & 0.524 & 0.588 & 0.539 & 0.811 & 0.593 & 0.650 & 0.572 & 0.815 & 0.612 & 0.666 & 0.583 \\
		rankGES & 0.788 & 0.495 & 0.561 & 0.522 & 0.806 & 0.576 & 0.636 & 0.564 & 0.810 & 0.595 & 0.652 & 0.573 \\
		%\hline
		%\hline
		ARGES & 0.780 & 0.446 & 0.489 & 0.786 & 0.799 & 0.535 & 0.576 & 0.773 & 0.803 & 0.555 & 0.595 & 0.764 \\
		rankARGES & 0.776 & 0.428 & 0.473 & 0.778 & 0.795 & 0.523 & 0.566 & 0.766 & 0.800 & 0.542 & 0.584 & 0.757 \\
		%\hline
		%\hline
		FCI+ & 0.837 & 0.589 & 0.671 & 0.652 & 0.865 & 0.684 & 0.755 & 0.720 & 0.871 & 0.702 & 0.771 & 0.732 \\
		%\hline
		%\hline
		LINGAM & 0.840 & 0.578 & 0.650 & 0.678 & 0.908 & 0.719 & 0.743 & 0.825 & 0.941 & 0.858 & 0.883 & 0.862 \\
		%\hline
		%\hline
		PC & 0.830 & 0.568 & 0.642 & 0.661 & 0.858 & 0.662 & 0.732 & 0.719 & 0.866 & 0.684 & 0.752 & 0.733 \\
		rankPC & 0.821 & 0.544 & 0.617 & 0.632 & 0.849 & 0.639 & 0.711 & 0.696 & 0.855 & 0.660 & 0.733 & 0.707 \\
		%\hline 
		%\hline 
		MMPC & 0.771 & 0.323 & 0.368 & 0.787 & 0.819 & 0.476 & 0.534 & 0.739 & 0.832 & 0.515 & 0.575 & 0.745 \\
		%\hline 
		%\hline
		MMHC & 0.800 & 0.495 & 0.557 & 0.579 & 0.820 & 0.570 & 0.625 & 0.633 & 0.826 & 0.587 & 0.642 & 0.647 \\
		%\hline 
		%\hline
		GS & 0.793 & 0.375 & 0.427 & 0.785 & 0.842 & 0.540 & 0.592 & 0.834 & 0.856 & 0.577 & 0.625 & 0.852 \\
    	%\hline 
    %	\hline
        IAMB & 0.745 & 0.316 & 0.390 & 0.705 & 0.815 & 0.510 & 0.574 & 0.794 & 0.835 & 0.556 & 0.614 & 0.821 \\
		%\hline 
		%\hline
		FastIAMB & 0.803 & 0.401 & 0.461 & 0.770 & 0.844 & 0.541 & 0.593 & 0.833 & 0.857 & 0.574 & 0.623 & 0.850 \\
		%\hline 
		%\hline
		IAMB-FDR & 0.783 & 0.325 & 0.372 & 0.825 & 0.837 & 0.523 & 0.578 & 0.815 & 0.850 & 0.564 & 0.613 & 0.843 \\
		%\hline 
		%\hline
	    PCI & 0.829 & 0.551 & 0.594 & \textbf{0.804} & 0.914 & 0.812 & 0.853 & 0.842 & 0.931 & 0.855 & 0.893 & 0.866 \\
		%\hline 
		%\hline
		Lasso & 0.870 & \textbf{0.729} & \textbf{0.812} & 0.732 & 0.889 & 0.778 & 0.848 & 0.773 & 0.893 & 0.786 & 0.854 & 0.780 \\
		\texttt{CORTH Features (Ours)} & \textbf{0.883} & 0.710 & 0.780 & 0.754 & \textbf{0.935} & \textbf{0.874} & \textbf{0.906} & \textbf{0.874} & \textbf{0.942} & \textbf{0.891} & \textbf{0.920} & \textbf{0.887} \\
		\bottomrule
		\end{tabular}
\end{table*}






==> TMLR 2022_ Causal Feature Selection via Orthogonal Search 2/tables_reg.tex <==
\begin{table*}[!ht]
    \footnotesize
	\caption[Caption for LOF]{\corrected{Performance across all the settings for different nonlinear probabilities. Each single entry in the table is averaged over 3750 simulations.}}
	\label{Table_reg_Nonlinear Probability}
	\centering
	\setlength{\tabcolsep}{4.12pt}
	\begin{tabular}{ l c c c | c c c | c c c| c c c} %@{\extracolsep{\fill}}
		\toprule
		& \multicolumn{12}{c}{Nonlinear Probability} \\
		\hline
		\multirow{2}{*}{Method} & \multicolumn{3}{c}{0} & \multicolumn{3}{c}{0.3} & \multicolumn{3}{c}{0.5} & \multicolumn{3}{c}{1} \\
		
		\multicolumn{1}{c}{} & TPR & CSI & F1 & TPR & CSI & F1 & TPR & CSI & F1 & TPR & CSI & F1\\
		\midrule
		%\hline
		%\hline
		Standard Regression & 0.149 & 0.103 & 0.139 & 0.166 & 0.112 & 0.141 & 0.175 & 0.108 & 0.136 & 1.000 & 0.801 & 0.801 \\
		%\hline
		%\hline
		Lasso & 0.237 & 0.116 & 0.176 & 0.285 & 0.126 & 0.202 & 0.360 & 0.165 & 0.263 & 1.000 & 0.046 & 0.046 \\
		%\hline
		%\hline
		Debiased Lasso & 0.238 & 0.117 & 0.178 & 0.267 & 0.112 & 0.178 & 0.300 & 0.124 & 0.202 & 1.000 & 0.050 & 0.050 \\
		%\hline
		%\hline
		Forward Stepwise Reg\_active & 0.174 & 0.112 & 0.162 & 0.157 & 0.110 & 0.167 & 0.194  & 0.129 & 0.190 & 1.000 & 0.329 & 0.329 \\
		%\hline
		%\hline
		Forward Stepwise Reg\_all & 0.04 & 0.039 & 0.060 & 0.062 & 0.059 & 0.085 & 0.089 & 0.086 & 0.116 & 1.000 & 0.861 & 0.861 \\
		%\hline
		%\hline
		LARS\_active & 0.073 & 0.054 & 0.094 & 0.104 & 0.078 & 0.131 & 0.118 & 0.081 & 0.134  & 1.000 & 0.382 & 0.382 \\
		%\hline
		%\hline
		LARS\_all & 0.017 & 0.016 & 0.028 & 0.030 & 0.029 & 0.048 & 0.039 & 0.037 & 0.057 & 1.000 & \textbf{0.866}  & \textbf{0.866} \\
		%\hline
		%\hline
		\texttt{CORTH Features (Ours)} & \textbf{0.481} & \textbf{0.287} & \textbf{0.407} & \textbf{0.436} & \textbf{0.258} & \textbf{0.366} & \textbf{0.364} & \textbf{0.220} & \textbf{0.313} & 1.000 & 0.610 & 0.610 \\
		\bottomrule
		\end{tabular}
\end{table*}


\begin{table*}[!ht]
    \footnotesize
	\caption[Caption for LOF]{\corrected{Performance across all the settings for different number of observation. Each single entry in the table is averaged over 3000 simulations.}}
	\label{Table_reg_Number of Observations}
	\centering
	\setlength{\tabcolsep}{4.12pt}
	\begin{tabular}{ l c c | c c | c c | c c | c c } %@{\extracolsep{\fill}}
		\toprule
		& \multicolumn{10}{c}{Number of Observations} \\
		\hline
		\multirow{2}{*}{Method} & \multicolumn{2}{c}{10} & \multicolumn{2}{c}{20} & \multicolumn{2}{c}{50} & \multicolumn{2}{c}{100} & \multicolumn{2}{c}{200} \\
		
		\multicolumn{1}{c}{} & CSI & F1 & CSI & F1 & CSI & F1 & CSI & F1 & CSI & F1\\
		\midrule
		%\hline
		%\hline
		Standard Regression & \textbf{0.250} & \textbf{0.250} & \textbf{0.250} & 0.250 & 0.250 & 0.250 & 0.263 & 0.272  & 0.392 & 0.499\\
		%\hline
		%\hline
		Lasso & 0.075 & 0.117 & 0.100 & 0.155 & 0.127 & 0.192 & 0.131 & 0.196 & 0.132 & 0.198 \\
		%\hline
		%\hline
		Debiased Lasso & 0.066 & 0.102 & 0.086 & 0.134 & 0.115 & 0.173 & 0.122 & 0.179 & 0.114 & 0.171 \\
		%\hline
		%\hline
		Forward Stepwise Reg\_active & 0.193 & 0.199 & 0.161 & 0.177 & 0.103 & 0.134 & 0.071 & 0.111 & 0.322 & 0.439 \\
		%\hline
		%\hline
		Forward Stepwise Reg\_all & 0.222 & 0.224 & 0.222 & 0.226 & 0.229 & 0.236 & 0.244 & 0.257 & 0.389 & 0.458 \\
		%\hline
		%\hline
		LARS\_active & 0.193 & 0.200 & 0.171 & 0.191 & 0.143 & 0.177 & 0.090 & 0.128 & 0.160  & 0.242 \\
		%\hline
		%\hline
		LARS\_all & 0.218 & 0.222 & 0.217 & 0.221 & 0.226 & 0.231 & 0.230 & 0.235 & 0.293 & 0.342 \\
		%\hline
		%\hline
		\texttt{CORTH Features (Ours)} & 0.125 & 0.173 & \textbf{0.250} & \textbf{0.314} & \textbf{0.353} & \textbf{0.445} & \textbf{0.443} & \textbf{0.548} & \textbf{0.550} & \textbf{0.640} \\
		\bottomrule
		\end{tabular}
\end{table*}

\clearpage

\begin{table*}[!ht]
    \footnotesize
	\caption[Caption for LOF]{\corrected{Performance across all the settings for different connectivities. Each single entry in the table is averaged over 5000 simulations.}}
	\label{Table_reg_sparsity}
	\centering
	\setlength{\tabcolsep}{4.12pt}
	\begin{tabular}{ l c c c | c c c | c c c } %@{\extracolsep{\fill}}
		\toprule
		& \multicolumn{9}{c}{Connectivity} \\
		\hline
		\multirow{2}{*}{Method} & \multicolumn{3}{c}{0.1} & \multicolumn{3}{c}{0.3} & \multicolumn{3}{c}{0.5} \\
		
		\multicolumn{1}{c}{} & TPR & CSI & F1 & TPR & CSI & F1 & TPR & CSI & F1 \\
		\midrule
		%\hline
		%\hline
		Standard Regression  & 0.395 & 0.267 & 0.290 & 0.372 & 0.292 & 0.313 & 0.350 & 0.284 & 0.310  \\
		%\hline
		%\hline
		Lasso   & \textbf{0.789} & 0.211 & 0.314 & 0.353 & 0.094 & 0.150 & 0.269 & 0.035 & 0.052 \\
		%\hline
		%\hline
		Debiased Lasso  & 0.787 & 0.211 & 0.314 & 0.296 & 0.054 & 0.087 & 0.270 & 0.037 & 0.055 \\
		%\hline
		%\hline
		Forward Stepwise Reg\_active   & 0.437 & 0.182 & 0.231 & 0.352 & 0.156 & 0.198 & 0.355 & 0.171 & 0.208 \\
		%\hline
		%\hline
		Forward Stepwise Reg\_all  & 0.356  & 0.315 & 0.343 & 0.275 & 0.235 & 0.252 &  0.263 & 0.234 & 0.245 \\
		%\hline
		%\hline
		LARS\_active  & 0.360 & 0.149 & 0.192 & 0.312 & 0.145 & 0.183 & 0.340 & 0.169 & 0.196 \\
		%\hline
		%\hline
		LARS\_all  & 0.289 & 0.246 & 0.264 & 0.267 & 0.233 & 0.246 & 0.259 & 0.231 & 0.239  \\
		%\hline
		%\hline
		\texttt{CORTH Features (Ours)}  & 0.494 & \textbf{0.367} & \textbf{0.417} & \textbf{0.540} & \textbf{0.274} & \textbf{0.355} & \textbf{0.677} & \textbf{0.390} & \textbf{0.499} \\
		\bottomrule
		\end{tabular}
\end{table*}

\begin{table*}[!ht]
    \footnotesize
	\caption[Caption for LOF]{\corrected{Performance across all the settings for different parameters for the Beta distribution. Each single entry in the table is averaged over 3000 simulations.}}
	\label{Table_reg_alpha_beta}
	\centering
	\setlength{\tabcolsep}{4.12pt}
	\begin{tabular}{ l c c | c c | c c | c c | c c } %@{\extracolsep{\fill}}
		\toprule
		& \multicolumn{10}{c}{Beta Distribution Parameters $(\alpha,\beta)$} \\
		\hline
		\multirow{2}{*}{Method} & \multicolumn{2}{c}{(0.5, 0.5)} & \multicolumn{2}{c}{(1, 3)} & \multicolumn{2}{c}{(2, 2)} & \multicolumn{2}{c}{(2, 5)} & \multicolumn{2}{c}{(5, 1)} \\
		
		\multicolumn{1}{c}{} & CSI & F1 & CSI & F1 & CSI & F1 & CSI & F1 & CSI & F1\\
		\midrule
		%\hline
		%\hline
		Standard Regression & 0.282 & 0.305 & 0.280 & 0.304 & 0.280 & 0.303 & 0.280 & 0.303  & 0.283 & 0.306 \\
		%\hline
		%\hline
		Lasso & 0.109 & 0.168 & 0.106 & 0.164 & 0.116 & 0.174 & 0.105 & 0.163 & 0.129 & 0.189 \\
		%\hline
		%\hline
		Debiased Lasso & 0.096 & 0.148 & 0.092 & 0.143 & 0.101 & 0.152 & 0.093 & 0.144 & 0.120 & 0.173\\
		%\hline
		%\hline
		Forward Stepwise Reg\_active & 0.169 & 0.211 & 0.168 & 0.210 & 0.169 & 0.211 & 0.172 & 0.214 & 0.172 & 0.215 \\
		%\hline
		%\hline
		Forward Stepwise Reg\_all & 0.261 & 0.279 & 0.257 & 0.275 & 0.265 & 0.284 & 0.259 & 0.278 & 0.266 & 0.284\\
		%\hline
		%\hline
		LARS\_active & 0.161 & 0.198 & 0.150 & 0.184 & 0.146 & 0.182 & 0.155 & 0.191 & 0.157 & 0.193 \\
		%\hline
		%\hline
		LARS\_all & 0.235 & 0.248 & 0.236 & 0.249 & 0.241 & 0.254 & 0.238 & 0.251 & 0.234 & 0.247 \\
		%\hline
		%\hline
		\texttt{CORTH Features (Ours)} & \textbf{0.336} & \textbf{0.417} & \textbf{0.330} & \textbf{0.411} & \textbf{0.354} & \textbf{0.434} & \textbf{0.336} & \textbf{0.417} & \textbf{0.363} & \textbf{0.441} \\
		\bottomrule
		\end{tabular}
\end{table*}

==> TMLR 2022_ Causal Feature Selection via Orthogonal Search 2/theorem_notation.tex <==
%repeating theorems

%%--------------
\newtheorem{theorem}{Theorem}
\newtheorem{acknowledgement}[theorem]{Acknowledgement}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{definition}[theorem]{Definition}
% \newtheorem{algorithm}[theorem]{Algorithm}
\newtheorem{axiom}[theorem]{Axiom}
\newtheorem{case}[theorem]{Case}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{conclusion}[theorem]{Conclusion}
\newtheorem{condition}[theorem]{Condition}
% \newtheorem{conjecture}[theorem]{Conjecture}
% \newtheorem{corollary}[theorem]{Corollary}
\newtheorem{criterion}[theorem]{Criterion}
% \newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{exercise}[theorem]{Exercise}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{notation}[theorem]{Notation}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{solution}[theorem]{Solution}
\newtheorem{summary}[theorem]{Summary}
\newtheorem{remark}{Remark}
%\newtheorem{corollary}{Corollary}
%\newtheorem{remark}{Remark}
% %-------------
% % \renewcommand{\text}[1]{{\mathrm{#1}}}
% \renewcommand{\text}[1]{{\textnormal{#1}}}

%%--------------
% \newcommand{\figref}[1]{{Fig.}~\ref{#1}}
% \newcommand{\secref}[1]{{Section}~\ref{#1}}
% \newcommand{\Secref}[1]{{Section}~\ref{#1}}
\newcommand{\tabref}[1]{{Table}~\ref{#1}}
\newcommand{\thref}[1]{{Theorem}~\ref{#1}}
%\newcommand{\algref}[1]{{Algorithm}~\ref{#1}}
\newcommand{\aref}[1]{{Algorithm}~\ref{#1}}
\newcommand{\propref}[1]{{Proposition}~\ref{#1}}
\newcommand{\lemref}[1]{{Lemma}~\ref{#1}}
\newcommand{\corref}[1]{{Corollary}~\ref{#1}}
\newcommand{\chref}[1]{{Chapter}~\ref{#1}}
\newcommand{\defref}[1]{{Definiton}~\ref{#1}}
